Exact Rate-Distortion in Autoencoders via Echo Noise

Compression is at the heart of effective representation learning. However, lossy compression is typically achieved through simple parametric models like Gaussian noise to preserve analytic tractability, and the limitations this imposes on learning are largely unexplored. Further, the Gaussian prior assumptions in models such as variational autoencoders (VAEs) provide only an upper bound on the compression rate in general. We introduce a new noise channel, \emph{Echo noise}, that admits a simple, exact expression for mutual information for arbitrary input distributions. The noise is constructed in a data-driven fashion that does not require restrictive distributional assumptions. With its complex encoding mechanism and exact rate regularization, Echo leads to improved bounds on log-likelihood and dominates $\beta$-VAEs across the achievable range of rate-distortion trade-offs. Further, we show that Echo noise can outperform flow-based methods without the need to train additional distributional transformations.

==> sections/_figs_.tex <==









\begin{figure}{\linewidth}
  \centering
  \includegraphics[scale = .65]{figs/rd_plots/rd_Omniglot200_zoom.pdf}
  \includegraphics[scale = .65]{figs/rd_plots/RECON_om_Omniglot200mmd_10.pdf}
  \vskip -.1in
    %\captionof{figure}{Omniglot Rate-Distortion and Visualization}
   %\label{fig:omni_rd}
\end{figure}

\clearpage



\begin{figure*}[htb]
%  figure placement: here, top, bottom, or page
  \centering
   \begin{subfigure}{\linewidth}
   \includegraphics[width=\linewidth]{figs/echo_200_final_nomc_64_1_EchoFSx_lld.pdf}
   %\label{fig:fx_a}
   \end{subfigure}  
   \begin{subfigure}{\linewidth}
   \includegraphics[width=0.5\linewidth]{figs/echo_200_final_nomc_64_1Fashion_MNIST_mi0133_1d_density.pdf}
    \end{subfigure}
   \begin{subfigure}{\linewidth}
   \includegraphics[width=0.5\linewidth]{figs/echo_200_final_nomc_64_1Fashion_MNISTtop_2d_density.pdf}
    \end{subfigure}
      %\caption{$f_j (\vx)$ vs. $s_j (\vx)$ for Fashion MNIST $\beta = 1$.  \textit{Top}:  The x-axis represents data points, sorted by likelihood.  The left column shows the two highest $I(X;Z_j)$ dimensions, while the right selects two low MI units, one saturated and one not.  \textit{Bottom Left:} Density plot of activations for bimodal dimension with MI = $0.133$. \textit{Bottom Right:} Joint density plot for high MI dimensions pictured above.}\label{fig:fxsx}
         \vskip -0.2in
\end{figure*}

\clearpage

\begin{figure*}[t]
\centering
%\%caption{Test Log Likelihood Bounds}
%\label{tab:elbos}
\small
\begin{tabular}{lccc}
%\toprule
 & \multicolumn{3}{c}{\textbf{Binary MNIST}} \\ \cmidrule(r){2-4}
Method & Rate &  Distortion & -ELBO  \\ \midrule
Echo 100 & 13.0 & \textbf{33.3}  & 46.3  \\
Echo 200 & \textbf{8.3} & 33.4 & \textbf{41.7} \\ \midrule 
%Echo1 fx MC & 30.5 & 62.5 & 93.0 \\ 
%Echo2 fx MC & 28.2 & 63.0 & 91.2 \\ \midrule
VAE & 25.8 & 68.8 & 94.6  \\
InfoVAE  & 33.2 &  64.8 & 98.1 \\ \midrule
IAF-MAF &  26.4 & 63.7 & 90.1  \\
Flow+MMD & 26.0 & 63.9 & \textbf{89.8} \\
\bottomrule
\end{tabular}
%\begin{tabularx}{.7\linewidth}{lccc}
\begin{tabular}{lccc}
%\toprule
 & \multicolumn{3}{c}{\textbf{Omniglot}} \\ \cmidrule(r){2-4}
Method & Rate &  Distortion & -ELBO  \\ \midrule
Echo 100 & 12.3 & \textbf{67.2 } & 79.5 \\
Echo 200 &\textbf{ 8.1} & 67.9 & \textbf{76.0} \\ \midrule
%Echo1 fx MC & 32.9 & 79.4 & \textbf{112.3} \\ 
%Echo2 fx MC & 32.3 & 80.9 & 113.2 \\ \midrule
VAE & 30.9 & 88.8 & 119.7 \\
InfoVAE & 35.0 & 86.4 & 121.5 \\ \midrule
IAF-MAF &  30.6 & 84.6 & 115.2  \\
Flow+MMD & 30.2 & 85.2 & 115.4  \\
\bottomrule
%\caption{Omniglot} \label{tab:omnielbo}
\end{tabular}
\begin{tabular}{lccc}
%\begin{tabularx}{.7\linewidth}{lccc}
%\toprule
 & \multicolumn{3}{c}{\textbf{Fashion MNIST}} \\ \cmidrule(r){2-4}
Method & Rate &  Distortion & -ELBO  \\ \midrule
Echo 100 &  11.1 & \textbf{206.6} & 217.7 \\
Echo 200 & \textbf{6.0} & 206.9 & \textbf{212.9} \\ \midrule
VAE & 14.7 & 221.6 & 236.3  \\ 
InfoVAE & 22.4 & 219.6 & 242.0 \\ \midrule
IAF-MAF & 16.2 &  218.3 & 234.5 \\
Flow+MMD &  15.7 & 218.0 & 234.7  \\
\bottomrule

%\caption{Fashion MNIST} \label{tab:fmnistelbo}
\end{tabular}
\end{figure*}




\clearpage
\begin{figure}[htb]
%  figure placement: here, top, bottom, or page
  \centering
   \includegraphics[scale = .5]{figs/2ds/echo2d_NOMC_2_1_2d_by_label.pdf}
    %\includegraphics[width=\linewidth]{figs/2ds/vae2d_2_1_2d_by_label.pdf}
       %\caption{Two-Dimensional $f(\vx)$ by Label:  Binary MNIST.  We obtain a total correlation $TC(Z) = 25.1$ for this distribution using the naive Gaussian estimator $-\log |\Sigma_{\mathrm{diag}}^{-1} \Sigma_{z}|$.} 
       %\label{fig:twod}
   \vskip -0.2in
\end{figure} 





\clearpage





\begin{figure}[htb]%  figure placement: here, top, bottom, or page
   \centering
   %\includegraphics[scale = .65]{figs/rd_plots/rd_BinaryMNIST200_new.pdf}
   \includegraphics[scale = .65]{figs/rd_plots/RECON_bm_BinaryMNIST200mmd_10.pdf}
   \vskip -0.2in
   %\caption{Binary MNIST Rate-Distortion and Visualization}
   \label{fig:bm_rd}
   \vskip -0.2in
\end{figure}

==> sections/_new_results.tex <==
\section{Additional Results}
\begin{table}[t]
\centering
\caption{Test Log Likelihood Bounds}
\label{tab:elbos}
\small
\begin{tabular}{lcccc}
%\toprule
 & \multicolumn{4}{c}{Binary MNIST} \\ \cmidrule(r){2-5}
Method & Rate & Dist & -ELBO & $\sigma$ \\ \midrule
Echo & 26.4 & 62.4 & \textbf{88.8} & \replaced{.18}{ .31} \\ \midrule  %& 26.2 & 62.3 & \textbf{88.3}
%Echo Rep & 27.0 & 62.9 & \textbf{88.9} & .19 \\ \midrule
%Echo+MMD & 26.0 & 62.5 & 88.5 \\ 
%Echo 64 &29.8  & 59.0 & 88.8 \\ \midrule
%Echo1 fx MC & 30.5 & 62.5 & 93.0 \\ 
%Echo2 fx MC & 28.2 & 63.0 & 91.2 \\ \midrule
VAE & 26.2 & 63.6 & 89.8 & .18 \\ % 144
InfoVAE & 26.0 & 64.0 & 90.0 & .14  \\ %& 26.9 & 66.0 & 92.9 \\ %\midrule %35.1 &  61.2 & 97.0 
VAE-MAF & 26.1 & 63.7 & 89.8  & .15 \\  % CHANGED
VAE-Vamp & 26.3 & 62.9 & 89.3 & .19 \\\midrule  % no norm & 26.0 & 68.4 & 94.4
IAF-Prior & 26.5 & 63.5 & \replaced{89.8}{ 90.0} & .13 \\     %26.6 & 62.7 & 89.3 \\ % no norm 
IAF+MMD & 26.3 & 63.6 & \replaced{89.9}{ 90.1} & \replaced{.15}{ .22}   \\ %89.9 w/base .   % no norm %<= no norm % 500 26.3 & 64.1 & 90.4
IAF-MAF & 26.4 & 63.6 & \replaced{89.7}{ 89.9} & .18  \\ % 
IAF-Vamp & 26.4 & 62.8 & 89.2 & .18  \\ % <=no norm % prev? & 26.4 & 63.7 & 90.1 
\bottomrule
\end{tabular}\hspace*{-0.1cm}%
\begin{tabular}{cccc} %\begin{tabularx}{.7\linewidth}{lccc}
%\toprule
 \multicolumn{4}{c}{Omniglot} \\ \cmidrule(r){1-4}
 Rate & Dist &  -ELBO & $\sigma$  \\ \midrule
 30.2 & 84.8 &  \replaced{114.4}{ \textbf{114.6}} &  \replaced{.30}{ .43} \\ \midrule %Echo
%Echo+MMD & 29.9 & 84.4 & \textbf{114.3} \\ 
% 64 & 32.5 & 80.5 & 113.0 \\ \midrule
%Echo1 fx MC & 32.9 & 79.4 & \textbf{112.3} \\ 
%Echo2 fx MC & 32.3 & 80.9 & 113.2 \\ \midrule
 30.5 & 86.5 & 117.0 & .44 \\ %VAE &  29.0 & 90.5 & 119.5
30.3 & 87.3 & 117.6 & .51 \\  %InfoVAE & no norm & 41.6 & 80.5 & 122.1  prev 37.0 & 84.1 & 121.1
30.5 & 86.4 & 116.9 & .31  \\ % vae maf
30.8 & 84.3 & 115.1 & .28 \\ \midrule % VAE-Vamp & 24.6 & 92.0 & 121.5 \midrule %VAE-MAF & %\midrule
 30.5 & 86.7 & 117.2 & .36 \\ % iaf prior
 30.7 & 86.4 & 117.1 & .15 \\ % .36 % IAF-mmd & no norm  % 30.2 & 86.6 & 116.8  %<= NORM GRAD IAF+MMD &
 30.6 & 86.5 & 117.1 & .24 \\ % norm! CORRECT IAF-MAF & 
 30.4 & 85.0 & 115.4 & .20 \\ %IAF-Vamp &
% 640x3 :   31.6 & 86.1 & 116.7 norm
\bottomrule % no norm 500 %IAF-Vamp & 29.8 & 87.9 & 117.7\\
%Flow+MMD & 30.2 & 85.2 & 115.4  \\
%\caption{Omniglot} \label{tab:omnielbo}
\end{tabular}\hspace*{-0.1cm}%     % \hspace*{0.1cm}% 
\begin{tabular}{cccc}
\multicolumn{4}{c}{Fashion MNIST} \\ \cmidrule(r){1-4}
Rate &  Dist & -ELBO & $\sigma$ \\ \midrule
16.6 & 218.3 & 234.9 & .21 \\ \midrule %Echo &
%Echo+MMD & 16.7 & 218.2 & 234.9 \\ \midrule
%Echo 64 &  & &  \\ \midrule
15.7 & 219.3 & 235.0 & .10  \\ % no norm?   & 226.0 VAE & 
15.6 & 219.5 & 235.1 & .10 \\ %\midrule %15.9 & 219.7 & 235.6 InfoVAE &
15.7 & 219.3 & 234.9  & .14 \\ % VAE MAF 
 15.9 & 218.5 & 234.4 & .06 \\ \midrule %VAE-Vamp & %VAE-MAF &  
15.8 & 219.1 & 234.9 & .10  \\ %IAF-Prior & 
15.6 & 219.2 & 234.9 & .13 \\ %IAF+MMD &
15.8 & 219.1 & 234.9 & .14 \\ %IAF-MAF &
16.0 & 218.3 & \textbf{234.3} & .16 \\  %IAF-Vamp 
%Flow+MMD &  15.7 & 218.0 & 234.7  \\
\bottomrule
%\caption{Fashion MNIST} \label{tab:fmnistelbo}
\end{tabular}%
\begin{tabular}{c} %\hspace*{0.2cm}% 
Params \\ \cmidrule(r){1-1}
($\cdot 10^6$) \\ \midrule
1.40 \\  \midrule 
1.40 \\ 
1.40 \\
3.12 \\
1.99 \\ \midrule
3.12 \\ 
3.12 \\ 
4.84 \\
3.71 \\  
\bottomrule
\end{tabular}
\end{table}




% \begin{table}[t]
% \centering
% \caption{All Modified Log Likelihood Bounds}
% \label{tab:elbos}
% \small
% \begin{tabular}{lcccc}
% %\toprule
%  & \multicolumn{4}{c}{Binary MNIST} \\ \cmidrule(r){2-5}
% Method & Rate & Dist & -ELBO & $\sigma$ \\ \midrule
% Echo & 26.4 & 62.4 & \textbf{88.8} & .31 \\ \midrule  %& 26.2 & 62.3 & \textbf{88.3}
% %Echo Rep & 27.0 & 62.9 & \textbf{88.9} & .19 \\ \midrule
% %Echo+MMD & 26.0 & 62.5 & 88.5 \\ 
% %Echo 64 &29.8  & 59.0 & 88.8 \\ \midrule
% %Echo1 fx MC & 30.5 & 62.5 & 93.0 \\ 
% %Echo2 fx MC & 28.2 & 63.0 & 91.2 \\ \midrule
% VAE & 26.2 & 63.6 & 89.8 & .18 \\ % 144
% InfoVAE & 26.0 & 64.0 & 90.0 & .28  \\ %& 26.9 & 66.0 & 92.9 \\ %\midrule %35.1 &  61.2 & 97.0 
% VAE-MAF & 26.1 & 63.7 & 89.8  & .15 \\  % CHANGED
% VAE-Vamp & 26.3 & 62.9 & 89.3 & .19 \\\midrule  % no norm & 26.0 & 68.4 & 94.4
% IAF-Prior & 26.1 & 63.7 & 89.8 & .24 \\     %26.6 & 62.7 & 89.3 \\ % no norm 
% IAF+MMD & 26.3 & 63.5 & 89.8 & .15   \\ %89.9 w/base .   % no norm %<= no norm % 500 26.3 & 64.1 & 90.4
% IAF-MAF & 26.1 & 63.6 & 89.7 & .21  \\ % 
% IAF-Vamp & 26.4 & 62.8 & 89.2 & .18  \\ % <=no norm % prev? & 26.4 & 63.7 & 90.1 
% \bottomrule
% \end{tabular}\hspace*{-0.1cm}%
% \begin{tabular}{cccc} %\begin{tabularx}{.7\linewidth}{lccc}
% %\toprule
%  \multicolumn{4}{c}{Omniglot} \\ \cmidrule(r){1-4}
%  Rate & Dist &  -ELBO & $\sigma$  \\ \midrule
%  30.2 & 84.8 & \textbf{114.6} & .43 \\ \midrule %Echo
% %Echo+MMD & 29.9 & 84.4 & \textbf{114.3} \\ 
% % 64 & 32.5 & 80.5 & 113.0 \\ \midrule
% %Echo1 fx MC & 32.9 & 79.4 & \textbf{112.3} \\ 
% %Echo2 fx MC & 32.3 & 80.9 & 113.2 \\ \midrule
%  30.5 & 86.5 & 117.0 & .44 \\ %VAE &  29.0 & 90.5 & 119.5
% 30.3 & 87.3 & 117.6 & .51 \\  %InfoVAE & no norm & 41.6 & 80.5 & 122.1  prev 37.0 & 84.1 & 121.1
% 30.5 & 86.4 & 116.9 & .31  \\ % vae maf
% & & & & \\ \midrule % VAE-Vamp & 24.6 & 92.0 & 121.5 \midrule %VAE-MAF & %\midrule
%  30.5 & 86.7 & 117.2 & .36 \\ % iaf prior
%  30.7 & 86.4 & 117.1 & .15 \\ % IAF-mmd & no norm  % 30.2 & 86.6 & 116.8  %<= NORM GRAD IAF+MMD &
%  30.6 & 86.5 & 117.1 & .24 \\ % norm! CORRECT IAF-MAF & 
%  30.4 & 85.0 & 115.4 & .20 \\ %IAF-Vamp &
% % 640x3 :   31.6 & 86.1 & 116.7 norm
% \bottomrule % no norm 500 %IAF-Vamp & 29.8 & 87.9 & 117.7\\
% %Flow+MMD & 30.2 & 85.2 & 115.4  \\
% %\caption{Omniglot} \label{tab:omnielbo}
% \end{tabular}\hspace*{-0.1cm}%     % \hspace*{0.1cm}% 
% \begin{tabular}{cccc}
% \multicolumn{4}{c}{Fashion MNIST} \\ \cmidrule(r){1-4}
% Rate &  Dist & -ELBO & $\sigma$ \\ \midrule
% 16.6 & 218.3 & 234.9 & .21 \\ \midrule %Echo &
% %Echo+MMD & 16.7 & 218.2 & 234.9 \\ \midrule
% %Echo 64 &  & &  \\ \midrule
% 15.7 & 219.3 & 235.0 & .10  \\ % no norm?   & 226.0 VAE & 
% 15.6 & 219.5 & 235.1 & .10 \\ %\midrule %15.9 & 219.7 & 235.6 InfoVAE &
% 15.3 & 222.3 & 236.6  & .45 \\ % VAE MAF 
%  15.9 & 218.5 & 234.4 & .06 \\ \midrule %VAE-Vamp & %VAE-MAF &  
% 15.8 & 219.1 & 234.9 & .10  \\ %IAF-Prior & 
% 15.6 & 219.2 & 234.9 & .13 \\ %IAF+MMD &
% 15.8 & 219.1 & 234.9 & .14 \\ %IAF-MAF &
% 16.0 & 218.3 & \textbf{234.3} & .16 \\  %IAF-Vamp 
% %Flow+MMD &  15.7 & 218.0 & 234.7  \\
% \bottomrule
% %\caption{Fashion MNIST} \label{tab:fmnistelbo}
% \end{tabular}%
% \begin{tabular}{c} %\hspace*{0.2cm}% 
% Params \\ \cmidrule(r){1-1}
% ($\cdot 10^6$) \\ \midrule
% 1.40 \\  \midrule 
% 1.40 \\ 
% 1.40 \\
% 3.12 \\
% 1.99 \\ \midrule
% 3.12 \\ 
% 3.12 \\ 
% 4.84 \\
% 3.71 \\  
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{Test Log Likelihood Bounds}
% \label{tab:elbos}
% \small
% \begin{tabular}{lcccc}
% %\toprule
%  & \multicolumn{4}{c}{Binary MNIST} \\ \cmidrule(r){2-5}
% Method & Rate & Dist & -ELBO & $\sigma$ \\ \midrule
% Echo & 26.4 & 62.4 & \textbf{88.8} & .31 \\ \midrule  %& 26.2 & 62.3 & \textbf{88.3}
% %Echo Rep & 27.0 & 62.9 & \textbf{88.9} & .19 \\ \midrule
% %Echo+MMD & 26.0 & 62.5 & 88.5 \\ 
% %Echo 64 &29.8  & 59.0 & 88.8 \\ \midrule
% %Echo1 fx MC & 30.5 & 62.5 & 93.0 \\ 
% %Echo2 fx MC & 28.2 & 63.0 & 91.2 \\ \midrule
% VAE & 26.2 & 63.6 & 89.8 & .18 \\ % 144
% InfoVAE & 26.0 & 64.0 & 90.0 & .28  \\ %& 26.9 & 66.0 & 92.9 \\ %\midrule %35.1 &  61.2 & 97.0 
% VAE-MAF & 26.1 & 63.7 & 89.8  & .15 \\  % CHANGED
% VAE-Vamp & 26.3 & 62.9 & 89.3 & .19 \\\midrule  % no norm & 26.0 & 68.4 & 94.4
% IAF-Prior & 26.5 & 63.5 & 90.0 & .13 \\     %26.6 & 62.7 & 89.3 \\ % no norm 
% IAF+MMD & 26.3 & 63.6 & 90.1 & .22   \\ %89.9 w/base .   % no norm %<= no norm % 500 26.3 & 64.1 & 90.4
% IAF-MAF & 26.4 & 63.6 & 89.9 & .18  \\ % 
% IAF-Vamp & 26.4 & 62.8 & 89.2 & .18  \\ % <=no norm % prev? & 26.4 & 63.7 & 90.1 
% \bottomrule
% \end{tabular}\hspace*{-0.1cm}%
% \begin{tabular}{cccc} %\begin{tabularx}{.7\linewidth}{lccc}
% %\toprule
%  \multicolumn{4}{c}{Omniglot} \\ \cmidrule(r){1-4}
%  Rate & Dist &  -ELBO & $\sigma$  \\ \midrule
%  30.2 & 84.8 & \textbf{114.6} & .43 \\ \midrule %Echo
% %Echo+MMD & 29.9 & 84.4 & \textbf{114.3} \\ 
% % 64 & 32.5 & 80.5 & 113.0 \\ \midrule
% %Echo1 fx MC & 32.9 & 79.4 & \textbf{112.3} \\ 
% %Echo2 fx MC & 32.3 & 80.9 & 113.2 \\ \midrule
%  30.5 & 86.5 & 117.0 & .44 \\ %VAE &  29.0 & 90.5 & 119.5
% 30.3 & 87.3 & 117.6 & .51 \\  %InfoVAE & no norm & 41.6 & 80.5 & 122.1  prev 37.0 & 84.1 & 121.1
% 30.5 & 86.4 & 116.9 & .31  \\ % vae maf
% & & & & \\ \midrule % VAE-Vamp & 24.6 & 92.0 & 121.5 \midrule %VAE-MAF & %\midrule
%  30.5 & 86.7 & 117.2 & .36 \\ % iaf prior
%  30.7 & 86.4 & 117.1 & .15 \\ % IAF-mmd & no norm  % 30.2 & 86.6 & 116.8  %<= NORM GRAD IAF+MMD &
%  30.6 & 86.5 & 117.1 & .24 \\ % norm! CORRECT IAF-MAF & 
%  30.4 & 85.0 & 115.4 & .20 \\ %IAF-Vamp &
% % 640x3 :   31.6 & 86.1 & 116.7 norm
% \bottomrule % no norm 500 %IAF-Vamp & 29.8 & 87.9 & 117.7\\
% %Flow+MMD & 30.2 & 85.2 & 115.4  \\
% %\caption{Omniglot} \label{tab:omnielbo}
% \end{tabular}\hspace*{-0.1cm}%     % \hspace*{0.1cm}% 
% \begin{tabular}{cccc}
% \multicolumn{4}{c}{Fashion MNIST} \\ \cmidrule(r){1-4}
% Rate &  Dist & -ELBO & $\sigma$ \\ \midrule
% 16.6 & 218.3 & 234.9 & .21 \\ \midrule %Echo &
% %Echo+MMD & 16.7 & 218.2 & 234.9 \\ \midrule
% %Echo 64 &  & &  \\ \midrule
% 15.7 & 219.3 & 235.0 & .10  \\ % no norm?   & 226.0 VAE & 
% 15.6 & 219.5 & 235.1 & .10 \\ %\midrule %15.9 & 219.7 & 235.6 InfoVAE &
% 15.3 & 222.3 & 236.6  & .45 \\ % VAE MAF 
%  15.9 & 218.5 & 234.4 & .06 \\ \midrule %VAE-Vamp & %VAE-MAF &  
% 15.8 & 219.1 & 234.9 & .10  \\ %IAF-Prior & 
% 15.6 & 219.2 & 234.9 & .13 \\ %IAF+MMD &
% 15.8 & 219.1 & 234.9 & .14 \\ %IAF-MAF &
% 16.0 & 218.3 & \textbf{234.3} & .16 \\  %IAF-Vamp 
% %Flow+MMD &  15.7 & 218.0 & 234.7  \\
% \bottomrule
% %\caption{Fashion MNIST} \label{tab:fmnistelbo}
% \end{tabular}%
% \begin{tabular}{c} %\hspace*{0.2cm}% 
% Params \\ \cmidrule(r){1-1}
% ($\cdot 10^6$) \\ \midrule
% 1.40 \\  \midrule 
% 1.40 \\ 
% 1.40 \\
% 3.12 \\
% 1.99 \\ \midrule
% 3.12 \\ 
% 3.12 \\ 
% 4.84 \\
% 3.71 \\  
% \bottomrule
% \end{tabular}
% \end{table}








% \begin{table}[h]
% %\begin{minipage}{\textwidth}
% %{.5\textwidth}
% \centering
% \caption{Disentanglement Scores}% (Independent Factors)}
% \begin{tabular}{llcccccc}
% \toprule % 4549351
% &  & \multicolumn{3}{c}{Full ($\perp$)} & \multicolumn{3}{c}{Dependent} \\ \cmidrule(r){3-5} \cmidrule(r){6-8} %\\ \midrule
%  &  & ELBO & FactorVAE & MIG & ELBO &  FactorVAE & MIG \\ \midrule 
% % \multirow{ 3}{*}{Echo LT} & $\beta = 1$ & 49.9  & 0.84 & \textbf{55.14 } & \\
% % %& $\beta = 4$ & 62.6 & 0.80 & 62.5 & 0.80 \\
% % & TC $\gamma = 20$ & 47.9 & 0.68 & & \\
% % %& 50.1 & 0.78 & 49.6 & 0.62 \\ % 51.4 & 0.77  \\
% % & TC $\gamma = 50$ & 47.9 & 0.63 & & \\ \midrule
% %&  51.2 & 0.68 & 54.0 & 0.81 \\ 
% \multirow{ 3}{*}{Echo} &$\beta = 1$ & 49.3 & 0.83 & 0.16 & 43.8 & 0.70 & 0.10 \\
% & $\beta = 4$ & 60.4 & 0.78 & 0.18 & 53.9 & 0.67 & 0.12 \\ 
% & $\beta = 8$ & 80.9 & 0.75 & 0.18 & 73.6 & 0.56 & 0.06\\ \midrule
% %& 55.2 & 0.69 & 76.5 & 0.55 \\ \midrule
% \multirow{ 3}{*}{VAE}  &$\beta = 1$ & 46.5 & 0.65 & 0.07 & 41.1 & 0.60 & 0.08 \\
% & $\beta = 4$ & 59.1 & 0.65 & 0.10 & 50.4 & 0.60 & 0.07 \\ 
% & $\beta = 8$ & 80.5 & 0.69 & 0.13 & 69.8 & 0.56 & 0.06 \\
%  \bottomrule
% \label{tab:disentanglement}
% \end{tabular}%
% \begin{tabular}{llcccccc}
% \toprule % 4549351
% &  & \multicolumn{3}{c}{Full($\perp$)} & \multicolumn{3}{c}{Dependent} \\ \cmidrule(r){3-5} \cmidrule(r){6-8} %\\ \midrule
%  & TC Reg & ELBO & FactorVAE & MIG & ELBO &  FactorVAE & MIG \\ \midrule 
% % \multirow{ 3}{*}{Echo LT} & $\beta = 1$ & 49.9  & 0.84 & \textbf{55.14 } & \\
% % %& $\beta = 4$ & 62.6 & 0.80 & 62.5 & 0.80 \\
% % & TC $\gamma = 20$ & 47.9 & 0.68 & & \\
% % %& 50.1 & 0.78 & 49.6 & 0.62 \\ % 51.4 & 0.77  \\
% % & TC $\gamma = 50$ & 47.9 & 0.63 & & \\ \midrule
% %&  51.2 & 0.68 & 54.0 & 0.81 \\ 
% \multirow{ 3}{*}{Echo} &$\beta = 1$ & & & & & &   \\
% & TC $\gamma = 20$ & 63.3 & 0.78 & 0.30 & 61.3 & 0.65 & 0.15 \\
% %& 49.6 & 0.81 & 52.7  & 0.77 \\
% & TC $\gamma = 50$& 71.9 & 0.79 & 0.30 & 80.6 & 0.58 & 0.16 \\ % 77, 88 = 83, .5 , .17
% & TC $\gamma = 100$& 76.8 & 0.77 & 0.29 & 85.9 & 0.57 & 0.12 \\\midrule % 91.67x2, .45, .14
% %& 55.2 & 0.69 & 76.5 & 0.55 \\ \midrule
% \multirow{ 3}{*}{VAE} &$\beta = 1$ & 46.5 & 0.65 & 0.07 & 41.1 & 0.60 & 0.08 \\
% %%& $\beta = 4$ & & & 59.2 & 0.71 \\
% & TC $\gamma = 20$ & 69.8 & 0.72 & 0.17 & 55.4 & 0.60 & 0.07 \\ %54.7 & 0.58 \\
% & TC $\gamma = 50$ & 71.3 & 0.73 & 0.18 & 59.9 & 0.53 & 0.07  \\
% & TC $\gamma = 100$ & 72.0 & 0.70 & 0.18 & 60.2 & 0.53  & 0.08 \\
%  \bottomrule
% \end{tabular} 
% %\end{minipage}%
% \end{table}



% old results text


%In contrast, any divergence from an independent Gaussian in a standard VAE would be penalized in the rate without adding information.
%These features stand in notable contrast to the vanilla VAE assumptions, which penalize the joint marginal divergence from an independent Gaussian and use a diagonal noise model.

% While Echo can learn dimensions with different mean and variance without penalty in the objective, we expect marginal flexibility has a relatively small impact in distinguishing our method.  Additionally, in App.\ref{app:tc}, we calculate a second-order approximation of total correlation to confirm that the noise is not independent across dimensions.
%We can calculate a second-order approximation of total correlation to show that the noise is not independent across dimensions (App.\ref{app:tc})


%We first seek to confirm several properties of the Echo noise described in Sec.~\ref{sec:echo_properties}.  We can calculate a second-order approximation of total correlation to show that the noise is not independent across dimensions (App.\ref{app:tc}).  In Appendix~\ref{app:marginals}, we visualize Echo marginal activations across individual dimensions, which are nearly Gaussian despite our lack of distributional assumptions.  


%Although Echo can learn dimensions with different mean and variance without penalty in the objective, these observations suggest flexibility in the marginal space is at most a minor factor distinguishing our method on the image datasets considered here.  The data-driven noise model and exact rate regularization throughout training remain as key elements of our approach to be evaluated.
%noiseobserve that the marginals learned by Echo are close to Gaussian despite its lack of distributional constraints. 


% In App.~\ref{app:marginals}, we visualize the noise and latent activations to show that Echo has the flexibility to learn marginals with different mean and variance without paying a cost in the objective.  Finally, we compare $f(\vx)$ and $S(\vx)$ across data points in App.~\ref{app:fxsx}, where Echo adds more noise on test examples for which the eventual model likelihood is low.

%can learn non-Gaussian marginals with different means and variances.  This flexibility does not come with a cost in the objective as it would for a VAE with prior assumptions.    %perhaps providing a useful quantity for anomaly detection or active learning.
%Although the Echo noise and output marginal can be non-Gaussian in general, we observe that the activations over latent dimensions appear surprisingly Gaussian in App.\ref{app:marginals}.  With this in mind, we can add an MMD penalty to the Echo marginal in the following sections to analyse the impact of marginal flexibility.  

%\textcolor{red}{Marginal gaussianity hypothesis testing ... previous results used a test which is ineffective with large number of samples.}%{Table \ref{tab:gaussianity}) evaluates the Gaussianity of individual marginal distributions using Shapiro-Wilks test \cite{shapirowilk}. For each model, we collect 2000 samples from the encoder for each test example as an estimate of the marginal.  We report the number of dimensions (out of 32), for which the Shapiro-Wilks test rejects the null hypothesis of the marginal being drawn from a Gaussian.  It is interesting to note that Echo may or may not learn primarily Gaussian marginals, while InfoVAE has the desired effect of enforcing Gaussianity in more dimensions than VAE.}
% \begin{table}[h]
% \parbox{.45\linewidth}{
% \centering
% \caption{Marginal Gaussianity Tests}
% \label{tab:gaussianity}
% \begin{tabular}{lccc}
% \toprule 
% Method & MNIST &  Omniglot & fMNIST  \\ \midrule
% Echo & 6 & 16 & \\
% VAE & 13 & 7 &  \\
% InfoVAE & 11 & 5 & \\ 
% \bottomrule
% \end{tabular}
% }\hfill
% \parbox{.45\linewidth}{
% \caption{Echo TC by Dataset}
% \label{tab:tc}
% \begin{tabular}{lccc}
% \toprule 
%     & MNIST &  Omniglot & fMNIST  \\ \midrule
% $TC(\mathcal{E})$ & 7.3 & 18.8 & 30.2 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

%\begin{table}[h]
%\centering


%Unless otherwise stated, we follow the implementation choices discussed in Sec. \ref{sec:implementation} for the Echo model, with $d_{max} = 199$ and batch size of 200.  See Appendix \ref{app:experiments} for further details on training and architectures. %and \ref{app:implementation} for more details on these choices.

%In order to explore the low rate limit, we set $\dmax$ equal to one less than the batch size, the maximum value it can take for sampling without replacement

%Unless otherwise stated, we use a $\tanh(\cdot/64)$ activation for $f(X)$ and a (log) sigmoid for $S(X)$, scaled according to $\dmax$ and float32 precision.  We set $\dmax$ equal to one less than the batch size, the maximum value it can take for sampling without replacement. 
%We use a batch size of 200 in Section \ref{sec:elboresults}, but discuss other choices in \ref{sec:rdresults}.  See Appendix \ref{app:experiments} for architecture and training details and \ref{app:implementation} for more details on these choices.





% We can visualize this in two dimensions in Figure \ref{fig:twod}, by plotting the activations of $Z$, which we have shown to have the same distribution as the noise $\bfeps$.  
% We can also show estimates of the total correlation $\kl[\qz || \prod q(z_j)]$ in a 64 latent factor model using the second-order covariance approximation. While this is only a lower bound on the true total correlation, we know that it is $0$ for conditionally independent Gaussian noise used in vanilla and Info-VAEs.



% \subsection{Understanding Echo Noise}

% \textbf{$f(\vx)$ and $S(\vx)$ by Dimension: \, \,} We first investigate the behavior of the shift and scale functions for Echo noise.  Using the fact that the mutual information in Equation \ref{eq:mi} decomposes into a sum over dimensions of $Z$ for diagonal $S(\vx)$, Fig. \ref{fig:fxsx} shows $f_j(\vx)$ and $s_j(\vx)$ across data points for dimensions with high and low mutual information.  
% We hypothesize that the model will attempt to preserve information on high likelihood examples. We observe this behavior in the top left latent factor, where, as likelihood increases, the magnitude of $f_j(\vx)$ increases and noise scaling $s_j(\vx)$ decreases.  This relationship is diminished or non-existent for low information or saturated dimensions.  





% The bottom left dimension of Fig. \ref{fig:fxsx} shows an interesting case where a bimodal latent factor has been learned, with additional visualization below.  While standard VAEs with Gaussian priors do not have the ability to model complex multi-modal posteriors, Echo should not suffer from such limitations.  Indeed, we see that joint distribution over the two most informative dimensions captures two distinct modes.
% %\textcolor{red}{RB: Input welcomed on how to interpret the bottom left.  This run also has particularly high TC... it's almost like it's working with another dimension?  will investigate examples if time permits}
% %width=\columnwidth
% %\begin{minipage}{\linewidth}


% %\end{minipage}
% % \begin{minipage}{\linewidth}
% % \begin{tabular}{lccc}
% % \toprule
% %  %& \multicolumn{3}{c}{Test} & Train \\ \cmidrule(r){2-4}
% % Method & Binary MNIST &  Omniglot & Fashion MNIST  \\ \midrule
% % Echo NoRep & 52.55 & 71.2 & 214.4  & \\
% % Echo Replace & 49.62 & 75.62 & 213.59 & \\
% % VAE & 94.56 & 119.71 & 236.35 & \\
% % InfoVAE &63.22 & 99.26 & 225.29 & \\
% % IAF & 90.09 & 115.14 & 234.75 & \\
% % IAF+MMD & 55.10 & 93.53 & 219.36 & \\
% % \bottomrule
% % \end{tabular}
% % \captionof{table}{Test $-$ELBO by Method and Dataset} \label{tab:datasetelbo}
% % \end{minipage} 

% \textbf{Correlated Noise: \, \,} \label{sec:corr_noise} The ability of the Echo model to add noise that is correlated across dimensions also distinguishes it from the common diagonal Gaussian conditional in VAEs.  We can quantify the divergence from independence for either the activations or the noise using the total correlation $TC(Z)$ or its conditional counterpart $TC(Z|X) = \kl[ q(\vz|\vx) || \prod q(z_j|\vx)]$, respectively \cite{watanabe}.  In particular, we show in Appendix \ref{app:tc} that $TC(Z) = TC(Z|X)$ for the case of diagonal $S(\vx)$, so that the dependence structure in the noise matches that of the eventual activations.

% While the joint density plot in Fig. \ref{fig:fxsx} also reflects this dependence, Fig. \ref{fig:twod} shows the V-like distribution of activations from an Echo model with two latent dimensions, colored by the label of the data sample.  We reiterate that this is equivalent to the noise distribution, with the training example simply specifying the first sample of a draw from the Echo noise $q(\bfeps)$. 

% Note that the conditional Gaussian noise model always has $TC(Z|X)=0$, with the activations likely having $TC(Z)>0$.  Previous works have used low $TC(Z)$ as a proxy for disentanglement (see, e.g. \cite{chen2018isolating}), but we leave further treatment of these quantities in Echo models for future work.
% %We leave further analysis of these quantities, including connections with the literature on disentanglement, for future work.

% %To briefly show that this quantity is nonzero for Echo noise, we naively estimate the total correlation of noise samples in a 64 latent factor model in Table \ref{tab:tc} using the second-order covariance approximation $TC(\bfeps) = -\log |\Sigma_{\mathrm{diag}}^{-1} \Sigma_{\bfeps} |$.



% % %\textcolor{red}{Unnecessary... we can easily sample the noise given encodings f(X), s(X)... calc on noise and validate in table} 
% %  %Our goal is to simply to show that these quantities are both non-zero for Echo, as there did not appear to be any meaningful relationship with either the rate or distortion in our models. Note, the conditional Gaussian noise model always has $TC(Z|X)=0$, with the activations likely having $TC(Z)>0$ (see, e.g. \cite{chen2018isolating}).  In Appendix \ref{app:tc}, we are able to show that $TC(Z) = TC(Z|X)$ for diagonal $S(\vx)$, but further examination of these quantities remains for future work.    
 
% % % \begin{table}[]
% % % \caption{TC by Dataset}
% % % \label{tab:tc}
% % % \begin{tabular}{lccc}
% % % \toprule 
% % %     & Binary MNIST &  Omniglot & Fashion MNIST  \\ \midrule
% % %  $TC(Z)$ & 26.2 & 16.8 & 43.0 \\
% % % \bottomrule
% % % \end{tabular}
% % % \end{table}
% % % \vskip -0.1in

==> sections/implementation.tex <==
\section{Implementation of Echo Noise Sampling}\label{sec:implementation}

Before proceeding to analyse results for the Echo noise channel, we first mention several implementation choices unique to our method.  In particular, we must ensure that the infinite sum defining the noise in Eq.\ref{eq:noise} converges and is precisely approximated using a finite number of terms. %  Further, for our mutual information expression to be valid, we need to be able to precisely sample the Echo noise using a finite number of terms %Numerically, Gaussian noise sampling can only be approximated to within machine precision and we discuss how to generate similarly accurate Echo samples. %In particular, we must ensure that the infinite sum defining the noise in Eq.\ref{eq:noise} converges.  Further, for our mutual information expression to be valid, we need to be able to precisely sample the Echo noise using a finite number of terms.  
%Numerically, Gaussian noise sampling can only be approximated to within machine precision and we discuss how to generate similarly accurate Echo samples.

%Just as we cannot exactly sample Gaussian noise and approximate it to within machine precision, we discuss how to generate Echo noise samples within machine precision.  

\textbf{Activation Functions: }  We parameterize the encoding functions $f(\vx)$ and $S(\vx)$ using a neural network and can choose our activation functions to satisfy the convergence conditions of Lemma \ref{condition}.  We let the final layer of $f$ use an element-wise $\tanh{(\cdot / 16)}$ to guarantee that the magnitude is bounded: $\forall \vx , \, |f(\vx)| \leq 1$.  We found it useful to expand the linear range of the $\tanh$ function for training stability, although differences were relatively minor and may vary by application.  It is also possible to clip the range of a linear activation to enforce a desired magnitude $|f(\vx)| \leq M$.

For the experiments in this paper, $S(\vx)$ is diagonal, with functions $s_j(\vx)$ on the diagonal.  We implement each $s_j(\vx)$ using a sigmoid activation, making the spectral radius $\rho(S(\vx)) = \max_j |s_j(\vx)| \leq 1$.  However, this is not quite enough to ensure convergence, as $\forall \vx, s_j(\vx) = 1$ would lead to an infinite amount of noise.  We thus introduce a clipping factor on $s_j(\vx)$ to further limit the spectral radius and ensure accurate sampling in this high noise, low rate regime.

\textbf{Sampling Precision: } When can our infinite sum be truncated without sacrificing numerical precision?  We consider the sum of the remainder terms after truncating at $\ell = \dmax$ using geometric series identities.  For $|f(\vx)| \leq M$ and $\rho(S(\vx)) \leq \rad$, we know that the sum of the infinite series will be less than $\frac{M}{1-\rad}$ . The first $\dmax$ terms will have a sum given by $M \big( \frac{1-\rad^{\dmax}}{1-\rad}\big)$, so the remainder will be less than $M \big( \frac{\rad^{\dmax}}{1-\rad}\big)$.  For a given choice of $\dmax$, we can numerically solve for $\rad$ such that the sum of truncated terms falls within machine precision $M \big( \frac{\rad^{\dmax}}{1-\rad}\big) \leq 2^{-23}$.  For example, with $M = 1$ and $\dmax = 99$, we obtain $\rad = 0.8359.$  We therefore scale our element-wise sigmoid to $s_j(\vx) = \rad \sigma(\cdot)$ for calculating both the noise and the rate.  

\textbf{Low Rate Limit: } \label{sec:clip}
This clipping factor limits the magnitude of noise we can add in practice, and thus defines a lower limit on the achievable rate in an Echo model.  For diagonal $S(\vx)$, the mutual information can be bounded in terms of $\rad$, so that $I(X;Z) = -\sum_{j=1}^{d_z} \mathbb E_q \log |s_j(\vx)| \geq -d_z \log \rad$.  Note that $\rad$ is increasing in $\dmax$, since considering more terms in the sum reduces the magnitude of remainder.  Each included term can then have higher magnitude, leading to lower achievable rates.  Thus, this limit can be tuned to achieve strict compression by increasing $\dmax$ or simply using fewer latent factors $d_z$. 

\textbf{Batch Optimization: } Another consideration in choosing $\dmax$ is that we train using mini-batches of size $B$ for stochastic gradient descent.  For a given training example, we can use the other iid samples in a batch to construct Echo noise, thereby avoiding additional forward passes to evaluate $f$ and $S$.  There is also a choice of whether to sample with or without replacement, although these will be equivalent in the large batch limit. In App.~\ref{app:additional}, we see little difference between these strategies, and proceed to sample without replacement to mirror the treatment of training examples. We let $\dmax = B-1$ to set the rate limit as low as possible for this sampling scheme.


% \textbf{Mean Centering: }  While it common to add  Gaussian noise centered at zero mean, we notice that Echo noise will not generally have this property since the mean of $f(\vx)$ is not constrained.  However, we can slightly adjust our channel to center the noise.  

% If we instead take $ \tilde{f}(\vx) \leftarrow f(\vx) - \mathbb{E}_\vx f(\vx)$, we can ensure that the Echo noise, which simply sums scaled versions of $ \tilde{f}$, will also be mean centered. For extra degree of freedoms, we can add a sample-independent shift parameter in each dimension $\mu = (\mu_1 \, ... \, \mu_{d_z})$ that does not affect either $H(Z)$ or $H(Z|X)$ by the translation invariance of entropy.  Our final channel can then be written $\vz = \mu + \tilde{f}(\vx) + S(\vx) \bfeps$, with $\bfeps$ constructed using $\tilde{f}$.


%We can slightly adjust the channel to enforce this property, obtaining several additional parameters in the process.

% In the case of diagonal $S(\vx)$, the mutual information in Eq.~\ref{eq:mi} simplifies to $\iq = -\sum_{j=1}^{d_z} \mathbb E_q \log |s_j(\vx)|$. Using the activation functions defined above, we can see that this leads to a lower bound on the achievable mutual information, $\iq \geq 23 \log 2 \cdot d_z / \dmax $.  Thus, achieving high compression requires using fewer latent factors or increasing $\dmax$.  The Echo channel requires high noise in this regime, so the value of $s_j(\vx)$ will approach saturating its upper limit and we must sample more terms from the sum to accurately reflect the noise.  
% %For the echo channel to achieve very low rates requires high noise and therefore more terms from the sum must be sampled.% For typical compression values and batch sizes we did not encounter this limit. Therefore, high compression requires increasing $\dmax$ to sample  %more terms from the infinite sum, or using fewer latent factors.

%$\frac{M}{1-\rad}$

% \textbf{Low Rate Limit:} 
% \section{Implementation of Echo Noise Sampling}\label{sec:implementation}
% Numerically, it is not possible to exactly sample Gaussian noise. Instead, we approximate Gaussian noise to within machine precision. For Echo noise, we discuss how to generate samples to within machine precision.

% Sampling the noise according to Eq.~\ref{eq:noise} requires an infinite sum, where each term requires a new sample drawn from the data distribution. With finite samples of data and computation, we are required to truncate this sum at $\ell = \dmax$. When can we do this without sacrificing numerical precision? We can look at the magnitude of the term that appears at $\ell = \dmax + 1$ for guidance. If $|f(\vx)| \leq M$ and we demand that the spectral radius, $\rho(S(\vx)) \leq K$, then the size of this remainder term is of the order $K^\dmax M$. For single precision floating point numbers, this will fall below machine precision if $K^\dmax M \leq 2^{-23}$, which implies that we can truncate our series at $\dmax$ as long as we set $M=1$ and $K = 2^{-23 / \dmax}$. For instance, for $\dmax = 100$, this would lead to a spectral radius bound of $K=0.852$.

% \textbf{Activation Functions: \quad} In practice, we parameterize the functions $f(\vx), S(\vx)$ using a neural network. We let the activation of the final layer of $f$ be an element-wise $\tanh{(\cdot / 64)}$. This guarantees that the magnitude of $f$ is bounded $|M| \leq 1$ and avoids heuristic clipping procedures. We also found it useful to expand the linear range of the $\tanh$ function.

% For the experiments in this paper, $S(\vx)$ is diagonal, with functions $s_j(\vx)$ on the diagonal. This makes the the spectral radius $\rho(S(\vx)) = \max_j |s_j(\vx)|$. To limit the spectral radius so that remainder terms are below machine precision, we set the activation function for $s_j(\vx)$ to be a scaled element-wise sigmoid, $2^{-23 / \dmax} \sigma(\cdot)$. 
% Conveniently, these choices also guarantee that we satisfy the conditions in Lemma~\ref{condition}. To reduce loss of numerical precision, we actually implement a function representing $\log s_j(\vx)$.%, which has the form of a constant minus a softplus function.
% % \ mean shift

% \textbf{Low Rate Limit: \quad} \ref{sec:clip}
% In the case of diagonal $S(\vx)$, the mutual information in Eq.~\ref{eq:mi} simplifies to $\iq = -\sum_{j=1}^{d_z} \mathbb E_q \log |s_j(\vx)|$. Using the activation functions defined above, we can see that this leads to a lower bound on the achievable mutual information, $\iq \geq 23 \log 2 \cdot d_z / \dmax $.  Thus, achieving high compression requires using fewer latent factors or increasing $\dmax$.  The Echo channel requires high noise in this regime, so the value of $s_j(\vx)$ will approach saturating its upper limit and we must sample more terms from the sum to accurately reflect the noise.  
% %For the echo channel to achieve very low rates requires high noise and therefore more terms from the sum must be sampled.% For typical compression values and batch sizes we did not encounter this limit. Therefore, high compression requires increasing $\dmax$ to sample  %more terms from the infinite sum, or using fewer latent factors.

% \textbf{Batch Optimization: \quad} Another reason it is important to limit $\dmax$ is that optimization is done with mini-batches using stochastic gradient descent. If we have $\dmax$ terms in each mini-batch, then we can use the other iid samples in a batch for sampling Echo noise. There is a choice of whether or not to sample with or without replacement from the batch. In the large batch limit, these will be equivalent, and in Appendix \ref{app:additional}, we see little difference between these strategies. We thus proceed to sample without replacement, mirroring the treatment of the data samples, and mean center the noise on a per-batch basis. 


==> sections/old/details_old.tex <==
\section{Echo Noise (with Sample-Dependent Scaling)}
\note{If this works out, I think we should just drop the simpler constant case altogether, in which case we don't have to mention sample dependent scaling as that is already naturally a part of VAE.}

\paragraph{VAE Encoder}
One of the key properties behind the success of variational auto-encoders is a scheme to sample from the encoder distribution in a tractable way that still allows analytic calculation of the regularization in the objective using the re-parametrization trick~\cite{kingma2013auto}. Let us recall how the encoder distribution, $q(z|x)$, is sampled.  
\begin{align}\label{eq:vae_sample}
z &= f(x) + s(x) \odot \epsilon \\ \nonumber
\epsilon &\sim \mathcal N(0,\mathbb I) \\\nonumber
\end{align}
In general, all variables can be vectors and $\odot$ is used to indicate component-wise multiplication of vectors. 
By defining the encoder distribution in this way, along with a ``prior'' distribution, $\pi(x)$ which is also standard normal, the following expressions can be calculated~\cite{kingma2013auto}. 
\begin{align}\label{eq:vae_reg}
\lefteqn{D(q(z|x) || \pi(z))} \\
&=  1/2 ~\mathbb E \left[\sum_j  \left(f_j(x)^2+s_j(x)^2  - \log(s_j(x)^2) - 1\right) \right] \nonumber 
\end{align}
\vskip -2.5em
\begin{align}
I_q(Z;X) &= D(q(z|x) || \pi(z)) - D(q(z) || \pi(z)) \nonumber \\
& \leq D(q(z|x) || \pi(z))  \label{eq:vae_mi}
\end{align}
\note{Rob, could you double check this?}
For VAEs, the term that appears as the regularizer is the KL divergence in the first line. However, in this work we adopt an information bottleneck style objective for which a compression term is the regularizer. In this case, the KL divergence is only an upper bound for the compression term. 
The close connection between the ELBO and the information bottleneck has been noted in several recent papers~\cite{}. 

\paragraph{Echo Encoder}
We now define a sampling scheme that can still be carried out efficiently and allows an analytic expression for the mutual information, instead of a bound. Moreover, we are not required to make assumptions about the form of the noise or prior being Gaussian, instead the noise distribution is an attenuated version of the inputs which we call ``echo noise''.  
\begin{align}\label{eq:echo_sample}
z &= f(x) + s(x) \odot \epsilon \\ \nonumber
\epsilon &= \sum_{\ell=0}^\infty \left(\bigodot_{\ell'=0}^{\ell-1} s(x^{(\ell')})\right) \odot f(x^\ell) \\ \nonumber
x^{(\ell)} &\overset{iid}{\sim} p(x)
\end{align}
The noise is constructed from the input distribution by repeatedly drawing iid samples and adding them together with attenuation by a factor $s(x)$. For this infinite series of echoes to die out, i.e., for the infinite sum to converge, we require that $\forall, j, x, ~~|s_j(x)| < 1$. 

Even though this echo noise sampling procedure does not allow us to analytically write down an expression for $q(z|x)$ or for $q(z)$, we can surprisingly still derive an exact analytic formula for the mutual information. 
\begin{align}\label{eq:echo_reg}
I_q(Z;X) &= - 1/2~ \mathbb E\left[\sum_j \log s_j(x)^2 \right]
\end{align}
This expression is derived in Sec.~\ref{sec:echo_proof}. While this exact expression for mutual information is simpler than the corresponding bound for VAEs in Eq.~\ref{eq:vae_mi}, the sampling procedure for the noise is more complex. We consider the implementation of echo noise sampling in Sec.~\ref{sec:implementation}.


\section{Implementing Echo Noise}\label{sec:implementation}
\note{Discussion of convergence of the series. Discuss the high noise, low MI limit, which is hard to handle. Show that the high MI limit is noiseless, $s(x)=0$. Discuss that $s(x)$ is calculated in the same way as for VAE. In fact, all architecture details are the same except for noise sampling. }

\section{Proof of Eq.~\ref{eq:echo_reg}}\label{sec:echo_proof}

Consider random variables $X$ drawn iid from a distribution, $p(x)$, and a noiseless encoder where we construct $Z=f(X)$, possibly parametrized by a neural network. To perform lossy compression, we include additive noise. The noise is attenuated by a data-dependent scaling factor, denoted with the random variable, $S=s(X)$, where $s(X)$ is also parametrized by a neural network. 
\benn
\bar Z = Z + S \odot \epsilon \qquad \epsilon\overset{iid}{\sim} q(\epsilon),
\eenn
The noise, $\epsilon$, is a random vector drawn from a distribution to be defined. Using the chain rule for mutual information, we have
\benn
I(\bar Z;X, Z, S) &= I(\bar Z;Z, S) + I(\bar Z;X|Z, S) \\
&= I(\bar Z; X) + I(\bar Z;Z,S|X).
\eenn
By the Markov assumptions of our graphical model, shown in Figure ~\ref{fig:encoder_new},  $I(\bar Z; X|Z, S) =0$. 
We also have $I(\bar Z; Z, S |X)=0$ since $Z, S$ are deterministic functions of $X$ and knowing them adds no new information if $X$ is already known. 
Therefore, we can write our lossy compression of $X$ as $I(\bar Z; X) = I(\bar Z; Z, S)$. Unfortunately, $I(\bar Z;Z, S)$ is still difficult to calculate, but we now show that the echo noise model makes it simple. 
 \begin{figure}[htb]%  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.5\columnwidth]{figs/proof2.pdf} 
   \caption{Graphical model of encoder with noise.}
   \label{fig:encoder_new}
   \vskip -0.1in
\end{figure}

The noise model could be specified by explicitly writing a parametric form for $q(\epsilon)$. Instead, we define this distribution implicitly through a sampling procedure. In particular, the noise looks like attenuated echoes of the encoding output $Z = f(X)$ obtained from i.i.d samples of the data distribution.  %The noise contribution of each successive sample trails off due to matrix exponentiation.
\begin{align*}
\epsilon &= \sum_{\ell=0}^\infty \left(\bigodot_{\ell'=0}^{\ell-1} s(x^{(\ell')})\right) \odot f(x^\ell) \\
x^{(\ell)} & \overset{iid}{\sim} p(x)
\end{align*}
%The superscripts label i.i.d. samples of $X$, but $D^\ell$ is just matrix exponentiation. 
A necessary condition for this procedure to be meaningful is that the series converges, which can be ensured by demanding that $\forall j,x\quad s_j(x) < 1$. We can ensure this by appropriately parametrizing the neural network defining $s(x)$. We define $q(\epsilon)$ to be the distribution that is consistent with this sampling procedure. 

Under this noise model, the distribution of $\bar Z$ has a special form. 
\benn
\bar Z &= f(X) + s(X) \odot \epsilon \\
\bar Z &= f(X) + s(X) \odot \sum_{\ell=0}^\infty \left(\bigodot_{\ell'=0}^{\ell-1} s(x^{(\ell')})\right) \odot f(x^\ell) \\
\bar Z &= \sum_{\ell=0}^\infty \left(\bigodot_{\ell'=0}^{\ell-1} s(x^{(\ell')})\right) \odot f(x^\ell) \\
\bar Z &\sim q(\epsilon)
\eenn
We have used the fact that the samples are i.i.d. to simply relabel the indices $X^{(\ell)}$ in the third line.  We see that the distribution over $\bar Z$ is identical to the noise distribution. 
We make use of this fact to derive the mutual information, $I(\bar Z; Z, S)=I(\bar Z; X)$. 
\be
I(\bar Z; Z, S) &= H(\bar Z) - H(\bar Z| Z, S) \nonumber\\
&= H(\epsilon) - H(Z + S \odot \epsilon | Z, S) \nonumber\\
&= H(\epsilon) - H(S \odot \epsilon | Z, S) \nonumber\\
&= H(\epsilon) - H(S \odot \epsilon | S) \nonumber\\ 
&= H(\epsilon) - H(\epsilon | S) - \sum_j \mathbb E \left[\log |S_j| \right]  \nonumber\\ 
I(\bar Z; X) &= -1/2 ~ \mathbb E_{x \sim p(x)} \left[\sum_j \log s_j(x)^2 \right] \label{eq:mi}
\ee
In the second line, we use the distributional equivalence between $\bar Z$ and $\epsilon$. The third line uses the invariance under translation for differential entropy. The fifth line uses the scaling rule for differential entropy, applied at every conditioned value of $S$. Since $\epsilon$ is independent of $S$, the two terms appearing in the fifth line cancel out. In the last line, we explicitly re-write the expression in terms of $x$ to highlight the similarity to the VAE regularizer. 
Note that no approximations are required. With this type of noise, we get an exact expression for the mutual information which, surprisingly, is \emph{independent of $p(x)$}. No matter the underlying data distribution, Echo noise constrains the mutual information.   Finally, this approach can easily extended to multiplicative noise, such as in \cite{informationdropout}.

\note{I think I should simplify by separately proving both terms $H(\bar Z) = H(\epsilon)$ and $H(\bar Z | Z, S)=H(\epsilon) + \ldots$. Then I can show more details for each part without it getting cumbersome. Especially that scaling step needs to be shown with more intermediate steps. }







% \section{Echo Noise}\label{sec:details}
% Having justified mutual information regularization from a compression perspective, we now introduce a noise model that admits an exact expression for this usually intractable term.


% \subsection{Derivation of the Echo Distribution}
% Consider a encoder where we take $Z=f(X)$, possibly parametrized by a neural network,  and perform compression by injecting additive noise
% \benn
% \bar Z = Z + U\epsilon \qquad \epsilon\overset{iid}{\sim} q_U(\epsilon),
% \eenn
% where $\epsilon$ is a random vector and $U$ is a matrix of parameters. Using the chain rule for mutual information, we have
% \benn
% I(\bar Z;X, Z) &= I(\bar Z;Z) + I(\bar Z;X|Z) \\
% &= I(\bar Z; X) + I(\bar Z;X|Z).
% \eenn
% By the Markov assumptions of our graphical model, shown in Figure ~\ref{fig:encoder},  $I(\bar Z; X|Z) =0$. \textcolor{red}{We also have $I(\bar Z; Z |X)=0$ since $Z$ is a sufficient statistic for $X$}. Therefore, we can write our lossy compression of $X$ as $I(\bar Z; X) = I(\bar Z; Z)$. Unfortunately, $I(\bar Z;Z)$ is still difficult to calculate, but we now choose a particular noise model that makes it simple. 
%  \begin{figure}[htb]%  figure placement: here, top, bottom, or page
%   \centering
%   \includegraphics[width=0.5\columnwidth]{figs/x_z.pdf} 
%   \caption{Graphical model of encoder with noise.}
%   \label{fig:encoder}
%   \vskip -0.1in
% \end{figure}

% The noise model could be specified by explicitly writing a parametric form for $q_U(\epsilon)$. Instead, we define this distribution implicitly through a sampling procedure. In particular, the noise looks like attenuated echoes of the encoding output $Z = f(X)$ obtained from i.i.d samples of the data distribution.  %The noise contribution of each successive sample trails off due to matrix exponentiation.
% $$
% \epsilon = \sum_{\ell=0}^\infty U^\ell f(X^{(\ell)}), \qquad X^{(\ell)} \overset{iid}{\sim} p(x)
% $$
% %The superscripts label i.i.d. samples of $X$, but $D^\ell$ is just matrix exponentiation. 
% A necessary condition for this procedure to be meaningful is that the series converges, which can be ensured by demanding the spectral radius of $U$ is less than one. In other words, the echoes should gradually die off as the series progresses. We define $q_U(\epsilon)$ to be the distribution that is consistent with this sampling procedure. 

% Under this noise model, the distribution of $\bar Z$ has a special form. 
% \benn
% \bar Z &= Z + U \epsilon \\
% \bar Z &= Z + U \sum_{l=0}^\infty U^\ell Z^{(l)} \\
% \bar Z &= U^0 Z + \sum_{l=0}^\infty U^{\ell+1} Z^{(l)} \\
% &= \sum_{l=0}^\infty U^\ell Z^{(l)}\\
% &\sim q_U(\epsilon)
% \eenn
% where we have used the fact that the samples are i.i.d. to simply relabel the indices $Z^{(l)}$.  We make use of this fact to derive the mutual information, $I(\bar Z; Z)=I(\bar Z; X)$. 
% \be
% I(\bar Z; Z) &= H(\bar Z) - H(\bar Z| Z) \nonumber\\
% &= H(\epsilon) - H(Z + U \epsilon | Z) \nonumber\\
% &= H(\epsilon) - H(U \epsilon | Z) \nonumber\\
% &= H(\epsilon) - H(U \epsilon) \nonumber\\ 
% &= H(\epsilon) - H(\epsilon) - \log \det U \nonumber\\
% I(\bar Z; X) &= -\log \det U \label{eq:mi}
% \ee
% In the second line, we use the distributional equivalence between $\bar Z$ and $\epsilon$. The third line uses the invariance under translation for differential entropy. The fifth line uses the scaling rule for differential entropy. 
% Note that no approximations are required. With this type of noise, we get an exact expression for the mutual information which, surprisingly, is \emph{independent of $p(x)$}. No matter the underlying data distribution, Echo noise constrains the mutual information.   Finally, this approach can easily extended to multiplicative noise, such as in \cite{informationdropout}.


% \subsection{Implementation}
% Echo noise can be easily inserted into autoencoder architectures in place of commonly used parametric noise models, at the computational cost of drawing additional samples.  We draw these samples from the same batch as is used for training, so that each $Z = f(X)$ both receives noise of its own and can contribute to the noise of other samples.  The number of samples is a hyperparameter to be tuned, although we did not observe particular sensitivity to its value.  We choose to take 50 samples for the Echo noise from a batch size of 100 in our experiments.

% In this work, we consider only the case where $U$ is a diagonal matrix.  In principle, $U$ could have more complex structure to introduce more nuanced noise, but calculating both the determinant and matrix exponentiation could become costly.  For example, the determinant is easy to calculate if $U$ is upper triangular, but it is not immediately clear how to speed up exponentiation.  

% Finally, to ensure that the higher order terms in our infinite noise series die out, we need to limit the maximum values in $U$.  In practice, we parametrize the diagonal elements $u_j$ by a sigmoid function to remain in the range $[0,1]$, so that the log determinant is simply $\sum_{j} \log u_j$.  Since the mutual information depends directly on the values $u_j$, we can update them using gradient descent as part of the rate-distortion objective.   

% However, it is interesting to note what may happen when $u_j$'s are close to 1.  In this case, the noise series may not truncate, so the samples beyond our finite range will still contribute to the noise.  In this case, the mutual information calculation will not be exact, as we are not able to add as much noise as the infinite series would prescribe.  We observe this behavior as the mutual information approaching a lower limit defined by the precision of the $u_j$ and number of Echo samples considered.


% %We sample the Echo noise within each batch. We have to limit the maximum value of $U$ so that higher order terms can be truncated in the infinite noise series. This is equivalent to lower bounding the mutual information. 
% %So far, we assume $U$ is diagonal. Though the determinant is still easy to calculate even if it is only upper triangular. However, calculating power of $U$ will be more time-consuming in that case.

==> sections/old/discussion.tex <==
\section{Discussion} \label{sec:discussion} 
% MOVED TO APPENDIX

%If the prior gives a loose likelihood bound, why do we use it?  Beyond the natural role of the prior in the generative model and Bayesian inference view of VAEs, we consider several possibilities for the common choice of an isotropic Gaussian prior $p(z) = \prod_{j=1}^{m} p(z_j) $, with $ p(z_j) \sim \mathcal{N}(0, 1) \, \forall j$.   
\textcolor{red}{should be moved back to VAE intro section?  too much discussion of this may detract from rate-distortion presentation} \\
In Section \ref{sec:prelim}, we have already mentioned several important considerations in jointly specifying an encoder $\enc$ and prior $\pz$ (or marginal approximation $r(\vz)$).  To what extent does our newly introduced Echo noise model respect these desirable properties or relax unnecessary assumptions?  We proceed by analysing the common choices of a conditionally independent Gaussian encoder and standard Gaussian prior.

\subsection{Encoder Considerations}

\textbf{Gaussianity:} The Gaussian assumption for each dimension of the encoder may limit our ability to model multi-modal posteriors and hurt performance in practice.  This has motivated flow-based methods such as \cite{rezende2015variational, kingma2016improved,papamakarios2017masked}, which apply a series of invertible transformations that preserve ease of sampling and analytic conditional density calculation. \\
% \textcolor{red}{Discuss echo after each of these?}

\textbf{Independence:} The conditional independence assumption of the encoder is rarely discussed in the literature, but Echo provides a mechanism for adding noise which is correlated across dimensions of the encoding.

\subsection{Marginal Considerations}
\textbf{Density Evaluation:}  The joint model density $p(\vz) \dec$ can be easily calculated with any simple parametric prior \textcolor{red}{or a flow-based marginal approximation such as }.  This can be useful for calculating importance weights such as in Importance Weighted Autoencoders \cite{burda2015importance} or evaluating generative models using a bound on mutual information \cite{alemi2018gilbo}. \\ % which calculates joint densities to re-weight samples and optimize a \textcolor{red}{different... or same bound but different dist} bound on likelihood.  \\

\textbf{Independence:}  The literature on `disentanglement' often operationalizes this goal in terms of statistical independence of the latent factors \cite{informationdropout, kim2018disentangling, chen2018isolating}.   \cite{informationdropout} argue that using a factorized prior \textit{encourages} independent $Z$. See Section \ref{sec: mi_terms} for further discussion.

However, the optimal factorized prior will still take the form of the true encoding marginals $\prod_j q_{\phi}(z_j)$, corresponding to additional regularization with the total correlation $\kl [ \qz || \prod_j q_{\phi}(z_j)]$.  This additional regularization may trade off performance for interpretability.   \\

\textbf{Sampling:} Since the prior is always easy to sample from, we can take unconditional samples from the generative model by simply feeding the result through the decoder $\dec$.

Any or all of these considerations may justify regularizing the encoding marginal $\qz$ to be close to a prior, particularly in cases where this prior can reflect domain knowledge or task-relevant structure \cite{lopez2018information}.  

%Nevertheless, it is important to separate the respective roles played by the two regularization terms in the ELBO: lossy compression via mutual information and marginal consistency with an assumed prior.

% \subsection{KL Divergence Calculations}

% analytic KL between gaussians \\
% flow models allow conditional density evaluation


\subsection{Mutual Information Terms} \label{sec:mi_terms}

\textcolor{red}{Analyse independence of latent variables for Echo noise}
Namely, for diagonal S, we have \\
$\iq$ = $\sum \limits_{j=1}^{M} I_q(X:Z_j)$\\
which implies $TC(Z) = TC(Z|X) >= 0$\\
(TC(Z|X) =0 for VAE)

==> sections/old/intro_old.tex <==


\section{Introduction}
A digital camera can record every bit of its sensory information to memory. A human exposed to the same visual information would be unable to recall or reconstruct the majority of perceived sensory data, but the tiny amount of information that is retained turns out to be extremely useful. While reproducing the compressive abilities of humans remains elusive, the mathematical problem of lossy compression has been formalized in rate-distortion theory. 

Rate-distortion theory frames lossy compression as a trade-off between storing bits about each input (rate) and retaining some measure of quality (distortion). Unfortunately, estimating the rate is itself a challenging, unsolved problem. \textcolor{red}{Standard approaches rely on heuristics and approximations to bound the rate in a way that is amenable to optimization. We introduce an alternate approach where we specify a particular form of noise, called echo noise, that allows us to analytically and exactly characterize the compression. }

%It has been observed that the generalization performance of deep neural networks is better than would be expected from theoretical arguments based on their complexity~\cite{rethinking_generalization}. It has been conjectured that intermediate layers of a network produce compressed representations of the inputs and that this leads to improved generalization~\cite{tishby_deep}. 
%While a formal link between compression and generalization has remained elusive, an intuitive argument is as follows. 
%The classical theory of PAC learning on discrete spaces shows that generalization error can be bounded by the logarithm of the size of the hypothesis class~\cite{haussler}. For representation learning, this means that if we could first compress our high-dimensional, continuous data into a small, discrete representation, we could improve the generalizability of predictions based on this representation. From an information-theoretic perspective, even if we do lossy compression in a continuous space, if the mutual information, $I(X;Z)$, is bounded, then there exists some discrete code for $Z$ that includes only $I(X;Z)$ bits on average and that contains as much information as our lossy representation~\cite{cover}. In other words, bounding mutual information restricts the complexity of our representation, and therefore should also improve generalization. 

%Despite the intuitive appeal of this argument, follow-up work has shown that, empirically, the generalization error for neural networks do not always benefit from compression \cite{saxe2018}. In particular, the details of the mutual information estimation scheme play a significant role. For this reason, we propose to compare a variety of methods for learning compressed representations to study how they affect generalization. 

%\Dan{I've added a section in blue containing a more direct bit about echo noise and its use. Feel free to not use any or all of it, but I thought I'd take a crack at it.}
Direct evaluation of mutual information is often intractable, with recent methods in the unsupervised learning literature resorting to variational approximations \citep{alemi2018fixing}, sampling \citep{phuong2018mutual}, or indirect optimization via other divergences \citep{infovae}.   The problematic term usually involves the marginal probability over the joint space of latent variables, which is alternatively treated as a prior in generative modeling approaches \citep{kingma2013auto,chen2016variational,tomczak2017vae}.  

In the present work, we instead construct the Echo noise model, which admits a closed form mutual information $I(X,Z)$ and can be dropped in as a replacement for the commonly used additive Gaussian noise layers.  While other models often assume noise is drawn independently across latent dimensions, Echo produces correlated noise which reflects the relationships in the output of an encoding function.  

Armed with this technique for exactly calculating mutual information, we further explore its utility as regularization for unsupervised learning models.  While previous works have made connections between latent variable modeling and the Information Bottleneck method \citep{informationdropout,alemi2016deep,alemi2018fixing,elidan2002information}, we present a more thorough justification in terms of rate-distortion theory \citep{cover} and highlight how previous assumptions and approximations can be better understood using this information theoretic approach.  Finally, we demonstrate how exact, direct mutual information regularization can \textcolor{red}{improve generalization from training to test error} by analyzing rate-distortion curves, which explore the frontier of feasible tradeoffs between compression and relevance.
   

We begin by reviewing the Variational Autoencoder framework in Section \ref{sec:prelim}, highlighting several simplifying assumptions which can severely limit performance.  In Section \ref{sec:echo}, we introduce the Echo noise model, which allows us to relax these assumptions while preserving their desired qualities and directly optimizing a tighter bound on log likelihood.  Further, the Echo model provides a simple, analytic form for the \textit{exact} mutual information between the data and latent variables, solidifying previous connections between representation learning and rate-distortion theory \cite{alemi2018fixing, achille}.    Armed with this noise model and mutual information regularization, we demonstrate state-of-the-art log likelihood estimates in Section \ref{sec:results} while also providing further intuition for our method.
   
   
%\subsection{Our Contribution}
% \textcolor{red}{We extend the rate-distortion analysis \cite{alemi2018fixing} by developing connections with the multivariate Information Bottleneck (MIB) \cite{friedman2001multivariate,elidan2002information}}.  We provide an \text{exact} characterization of the compression term, or information rate $I_q(X;Z)$, by introducing the new Echo noise model.  Finally, we demonstrate that this mutual information regularization can improve generalization from training to test set and reduce over-fitting when learning from limited data.  

%Intended as a replacement for the now standard Gaussian layer, the use of our proposed distribution greatly simplifies Mutual Information-based regularization and compression. We present the analytic derivation of Echo Noise as well as its closed form mutual information property, its computational implementation and relevant parameters, and then present empirical results on its use in standard tasks as compared to equivalent Gaussian noise models. }


%\BlueComment{Current methods often rely on the computation of mutual information terms $I(X,Z)$. While this is analytically useful, practically it implies computing entropic terms such as $KL[~p(Z|X)~|~p(Z)~]$. Direct evaluation is usually either unstable, intractable, or both; current state of the art approximates these values using either sampling or loose upper bounds \CiteNeeded \CiteLater{Maybe worst case cite ourselves using jensens?}. \Dan{(Or Heuristics?)}



==> sections/old/preliminaries_old.tex <==
% Moved and consolidated material in rd.tex

\section{Variational Autoencoders} \label{sec:prelim}
Many modern approaches to unsupervised representation learning seek to maximize the marginal likelihood of the data under a generative model with latent variables.    Often, we assume a prior distribution $p(\vz)$ over latent variables $Z = \{z_1, ... z_j, ... z_M\}$ and model the data using a decoder $p_{\theta} (\vx|\vz)$  parametrized by a deep neural network.  However, maximum likelihood estimation of these parameters is usually intractable, as the 
data marginal $p_{\theta}(\vx) = \int p(\vz) \dec d{\vz}$ involves a high dimensional integral over $Z$.    

Variational Autoencoders (VAEs) \cite{kingma2013auto,rezende2014stochastic} utilize two key components to circumvent this problem.   First, the Evidence Lower Bound (ELBO) objective provides a tractable lower bound on the likelihood.  Instead of integrating over $p(\vz)$, the ELBO instead takes expectations with respect to the data distribution and a learned encoding distribution $q_{\phi}(\vz|\vx)$.  The gap in the lower bound reflects the difference between the `true' posterior $p_{\theta}(\vz|\vx)$ and our posterior approximation $q_{\phi}(\vz|\vx)$.
%although good ELBO values do not necessarily reflect accurate posterior inference \cite{infovae}  
% approximate / amortized posterior inference 
\benn
\eq \log \lld & \geq  \eq \log p(\vx)  - \kl [ \enc   || p_{\theta}(\vz|\vx)) ] \\
\mathcal L_{\text{ELBO}} & = \eq \log \dec - \kl [ \enc || p(\vz)]  %\label{eq:elbo} %_{q(\vx, \vz)}
\eenn
A second key property of VAEs, the reparametrization trick, defines a procedure for sampling from the encoding distribution that is amenable to gradient optimization.  In particular, we assume a parametric distribution $\enc$, sample an auxiliary noise variable $\bfeps$, and transform it using a set of differentiable functions, e.g. $g_{\phi} (\vx) = \{ f(\vx), S(\vx) \}$\footnote{Note, we will usually omit the dependence of $f(\vx)$ and $S(\vx)$ on $\phi$ in what follows}.  For example, with a conditionally independent Gaussian encoder, we can write:
\be
\vz & = f (\vx) +  S(\vx) \odot \bfeps \label{eq:enc} \\
& \bfeps \sim \mathcal{N}(0 , \mathbb{I}_M) \\
& S(\vx) \triangleq diag(s_{j}(\vx))
\ee
%This allows for fast sampling from the approximate posterior and.  
This reparametrization means we can take empirical expectations of the first term of Equation \ref{eq:elbo}, while still obtaining unbiased, low variance gradient estimates.  Further, the distribution for the encoder is usually chosen to admit a tractable form for the second term, a KL divergence to the prior.  However, these parametric assumptions are clearly linked, as the commonly-used analytic expression for the KL divergence relies on \textit{both} $\enc$ and $\pz$ being Gaussian.  We will revisit the potential impact of these assumptions in Section \ref{sec:details}.


\subsection{Likelihood Bounds}
While the prior $\pz$ has a natural interpretation in the Bayesian inference and generative approaches to latent variable modeling, how does it affect our goals of maximum likelihood learning?  

As in \cite{elbosurgery}, we can further decompose the KL divergence regularization term by considering the true marginal $\qz$ induced by the encoder :
\benn
\kl [ \enc || p(\vz) ] & = && \kl [ \enc || \qz ] \\
&   && + \kl [ \qz || p(\vz) ] \\
& = && \iq  +\kl[ \qz || p(\vz) ]
\eenn
This decomposition lends insight into the orthogonal goals of the traditional ELBO regularization term.  The mutual information $\iq$ encourages \textit{lossy compression} of the data into a latent code, while the marginal KL divergence enforces consistency with the generative model prior.   The non-negativity of the KL divergence implies that each of these terms detracts from our bound on log likelihood.
\be
\mathcal L_{\text{ELBO}} &= \eq \log \dec - && \kl [ \enc || \qz ] \\
&  - &&\kl [ \qz || p(\vz)] \\
& \leq \eq \log \dec - && \kl [ \enc || \qz ] \label{eq:tigher}
\ee
As shown in Appendix \ref{sec:appendix_marginal}, the true marginal $\qz$ is in fact the minimizer $ \argmin_{r} \kl [ \enc || r(\vz) ]$ among all distributions over $Z$, also known as the $m$-projection in information geometry \cite{}.  Any other marginal $r(\vz)$ will incur an approximation error of $\kl [ \qz || r(\vz)]$.  A static prior can thus be seen as providing a particular and likely loose marginal approximation \cite{gao2018auto, alemi2018fixing}.  Indeed, the analysis in \cite{rosca2018distribution} shows that the marginal divergence often dominates the mutual information, even for flow-based encoders or adversarial approaches and particularly for difficult datasets.

Several VAE extensions have observed this fact and considered `learned' priors \cite{chen2016variational, tomczak2017vae} or flow-based approximations \cite{alemi2018fixing} that seek to match $\qz$, thereby reducing $\kl [ \qz || r(\vz)]$ and tightening the ELBO.  In the absence of any domain-specific structure encoded in these priors or marginal approximations, we advocate focusing only on the lossy compression goal of variational autoencoding.  From this perspective, these approaches can be seen as providing upper bounds on the true quantity of interest, $\iq$.


%Our approach is slightly different.  Instead of using a diagonal covariance for the noise distribution, we could imagine sampling $\bfeps$ from a multivariate Gaussian $\Sigma_{\bfeps}$ with more complex (possibly learned) structure.  Since $g_{\phi} (\vx, \bfeps)$ is a deterministic transformation, the encoder would also be multivariate Gaussian, relaxing the conditional independence assumption above.  Evaluating $\kl [ \enc ||  p(\vz) ]$ now involves taking the determinant of $\Sigma_{\bfeps}$, but can still be done in closed form.   \textcolor{red}{While this scheme is implemented as a baseline in Section \ref{sec:results}}, our proposed method extends the intuition of introducing correlation into the noise distribution.  However, in a similar spirit to \cite{correlated_vae}, we instead induce this correlation across \textit{data points} rather than noise dimensions.



==> sections/old/related_old.tex <==
\section{Related Work}\label{sec:related_old} 

\subsection{Rate Distortion Theory}
Our work most closely aligns with the variational bounds on mutual information in \cite{alemi2018fixing} and the (supervised) Information Bottleneck principle \cite{tishby2000information, informationdropout, alemi2016deep}.  These interpretations emphasize the compression ability the encoding function, and the important quantity to regularize is the mutual information.  

The Information Bottleneck principle can be seen as a special case of rate-distortion theory


\subsection{Unsupervised Learning}
A number of recent works have argued that the maximum likelihood objective may be insufficient to learn "useful" or "interesting" representations of data \cite{alemi2018fixing,phuong2018mutual}.  In particular, when paired with powerful decoders that can match the data distribution, Variational Autoencoders (VAEs) may learn to completely ignore the latent code \cite{bowman2016}.  Adding mutual information terms or constraints to the objective function is commonly proposed as a solution \cite{infovae,phuong2018mutual,braithwaite2018bounded,alemi2018fixing}, although justification for these objectives vary.  Further, since mutual information is intractable in general, previous works have resorted to myriad different approximations, including through sampling \cite{phuong2018mutual}, density estimation with autoregressive flow models\citep{papamakarios2017masked,kingma2016improved,germain2015made}, or indirectly optimization via other divergences \cite{infovae}.

In particular, the infoVAE model of \cite{infovae} provides an interesting, more direct comparison to our Echo method.  
\textcolor{red}{ELBO + big MMD penalty} \\
MMD penalty $\implies \qz \approx \pz$, so that $\kl [\enc || \pz] \approx \iq$
%\textcolor{red}{many estimators focus on empirical sample mixture distribution... sources of disentanglement, artemy}


A standard approach in unsupervised learning is to assume a generative model and maximize the likelihood of the data or its tractable Evidence Lower Bound (ELBO):
\begin{align*}
\mathcal L = \mathbb{E}_{q} \log p(\vx) & \geq  \mathbb{E}_{q} \log p(\vx)  - D_{KL} [  q(\vz|\vx) || p(\vz|\vx) ] \\
\mathcal L_{\text{ELBO}} & = \mathbb{E}_{q(\vx, \vz)} \log p(\vx|\vz) - D_{KL} [q(\vz|\vx) || p(\vz)] 
\end{align*}
where the expectation reflects reconstruction ability, and the second term serves as a regularizer.  By considering the true marginal $q(\vz)$,  we can instead decompose this KL divergence into $D_{KL}[ q(\vz|\vx) || p(\vz) ] = D_{KL}[ q(\vz|\vx) || q(\vz) ] + D_{KL}[ q(\vz) || p(\vz) ] $ \citep{elbosurgery} and obtain
\begin{alignat*}{2}
\mathcal L_{\text{ELBO}} &= \mathbb{E}_{q(\vx, \vz)} \log p(\vx|\vz) && - D_{KL}[q(\vz|\vx) || q(\vz)] \\
& && - D_{KL}[q(\vz) || p(\vz)] \\
& \leq \mathbb{E}_{q(\vx, \vz)} \log p(\vx|\vz) && -  D_{KL}[q(\vz|\vx) || q(\vz)]
\end{alignat*}
With the appearance of the mutual information $I_q(X;Z)$, the first two terms can be identified as a rate-distortion optimization with distortion measure $d(\vx, \vz) = -\log p(\vx|\vz)$.  


This motivation of latent variable modeling as a relevant compression problem sidesteps the need for a prior, and provides a tighter bound on log likelihood in the process.  Although estimating the mutual information regularization term may still be intractable, it is natural to consider training variational approximations of the marginal
\begin{align}
\mathbb{E}_{q(\vz)} \log q(\vz) = \sup_{r(\vz)} \mathbb{E}_{q(\vz)} \log r(\vz) \label{eq:mlmarginal}
\end{align}
Several recent works have analyzed the resulting upper bound on mutual information,
\begin{align*}
D_{KL} [ q(\vz|\vx) || q(\vz)] \leq D_{KL} [ q(\vz|\vx) || r(\vz) ]
\end{align*}

\citet{alemi2018fixing} discuss this quantity as the rate, while \citet{chen2016variational} argue that learning the prior reduces coding inefficiency from a bits back perspective \citep{Hinton1993bitsback}.  Marginal approximations such as autoregressive flow models \cite{papamakarios2017masked} or the VampPrior \citep{tomczak2017vae} then are trained to maximize the likelihood of samples from the encoder output as in Equation \ref{eq:mlmarginal}.  

 
% derivations from the en
%The intractable term in the mutual information involves the marginal distribution over the joint latent space.  From a generative modeling perspective, this is often treated as prior $p(\vz)$
%This intractable term involving the joint latent space has been analyzed from both the generative and compression perspectives.  \cite{tomczak2017vae} observe that the optimal value for a generative prior in the ELBO is the "aggregated posterior" of the encoder  $q_(\vz).$, which is made explicit by the decomposition of \cite{elbosurgery} in Equation \eqref{eq:elbosurgery}.  Finally, \cite{chen2016} argue that learning this prior improves coding efficiency using a bits-back argument, providing an information-theoretic view of the generative process which complements our encoding focus.

%In this sense, our work most closely aligns with the variational bounds on  mutual information in \cite{alemi2018fixing} and the (supervised) Information Bottleneck principle \cite{tishby2000information, informationdropout, alemi2016deep}.  Under these interpretations, we emphasize the compression ability of our encoder, and the important quantity to regularize is the mutual information.  The isotropic Gaussian prior commonly used in VAEs can then be viewed as a particular, inflexible marginal approximation, likely providing a loose upper bound on the true $I_q(X;Z)$ \cite{gao2018auto}.  
%\footnote{This mapping is not injective if the $R(D)$ function is not strictly convex, which means $\beta$ cannot explore the optimal frontier. Optimizing using a constant $D$ may be preferable in these cases. See \citep{alemi2018fixing, kolchinsky2018pathologies} for discussion.}



%A number of works have proposed the $\beta$-VAE objective \cite{betavae}, most convincingly through arguments relating it to the Information Bottleneck method \cite{tishby2000information, informationdropout, alemi2016deep}.

% \cite{zhao2018lagrangian} intriguingly propose optimizing Lagrange multipliers which enforce `consistency' constraints on $q(\mathbf{x}, \mathbf{z})$ and $p(\mathbf{x}, \mathbf{z})$,
% %with respect to constraints on the ELBO and divergence between $q(z)$ and $p(z)$, 
% but our current understanding nonetheless requires target values for these constraints to be `leaked' to the model \cite{zhao2018lagrangian,alemi2018fixing}. 

%CorEx~\citep{corex,corex_theory,sieve}
 

==> sections/old/results_old.tex <==
\section{Results}\label{sec:results}
%To demonstrate the impact of exact mutual information regularization on generalization ability, we plot rate-distortion curves on both the train and test set for models trained at various parameters values $\beta$.  We compare an autoencoder with additive Echo noise to a standard VAE with additive Gaussian noise, along with an autoencoder with inverse autoregressive flow in the encoder \cite{kingma2016improved} and an autoregressive flow marginal approximation \cite{papamakarios2017masked}.  

We begin by validating several theoretical hypotheses above in order to more fully understand the new Echo noise distribution.  We also demonstrate greatly improved test log-likelihood bounds compared to infoVAE and standard VAEs on a variety of datasets.



%For supervised learning, the information bottleneck. 
%$$ \max_{\bar Z = f(x) + D \epsilon} I(\bar Z; Y) - \beta I(X;\bar Z)$$
%For unsupervised learning, use CorEx / VAE.
%$$ \max_{\bar Z = f(x) + D \epsilon} \sum_i I(X_i ; \bar Z) - \beta I(X;\bar Z)$$

%Some preliminary experiments

\subsection{Understanding Echo Noise}
\textcolor{red}{Correlations in 2-d MNIST space} \\
\textcolor{red}{Level sets of echo noise added} \\


many samples from same echo f(x), s(x) fed through decoder (uninteresting...)

\begin{figure}[htb]%  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.7\columnwidth]{figs/echo_fig.pdf} 
   \caption{Examples of Additive Echo Noise}
   \label{fig:echo_fig}
   \vskip -0.1in
\end{figure} 



\subsubsection{MNIST, 2-D latent space}
 \begin{figure}[htb]%  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.4\columnwidth]{figs/latent2.png}  
   \caption{Distribution in 2-d latent space.}
   \label{fig:latent}
   \vskip -0.1in
\end{figure}

\subsubsection{MNIST, 2-D latent space}
 \begin{figure}[htb]%  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.7\columnwidth]{figs/manifold2.png} 
   \caption{Manifold in 2-d latent space.}
   \label{fig:manifold}
   \vskip -0.1in
\end{figure} 
 

\subsection{Estimating Echo Mutual Information with Autoregressive Models}

\textcolor{red}{Idea: train a density estimator on the encoding activations, shuffle activations (for TC), and noise samples} \\

confirm estimate of I(X:Z) and that noise = encoding \\

estimate TC(Z) = T(Z|X) > 0 \\
\textcolor{red}{VAE results = MI = 0 ?!?}


\subsection{ELBO Evaluation}

We use the same convolutional architecture as in \citep{alemi2018fixing} on the static binarized MNIST \citep{salakhutdinov2008quantitative} and Fashion MNIST datasets \citep{xiao2017}. 


We find that optimizing both the KL divergence and MMD terms in InfoVAE provides remarkably better ELBO values than a vanilla VAE.  This appears to have gone unnoticed in \cite{infovae}, which reports the ELBO for a model trained with \textit{only} MMD regularization.


\subsubsection{MNIST}

\subsubsection{fMNIST}


\subsubsection{Penn Machine Learning Benchmark}

\textcolor{red}{debugging}


\subsection{Other Performance Evaluations}
\textcolor{red}{Sensitivity of ELBO performance to size of latents} \\

\textcolor{red}{activation for f(x):} linear, relu, scaled tanh, sigmoid for f(x)
\textcolor{red}{note: also allows us to bound f(x) and ensure noise within machine precision}


\textcolor{red}{activation for s(x):}tanh, sigmoid for s(x)


==> sections/rd.tex <==
\section{Connections With Rate-Distortion Theory}\label{sec:rd}
%\subsection{}
Having presented a method for exact calculation of $\iq$ and shown how this quantity can lead to a tighter bound on likelihood, we now draw connections to rate-distortion theory within the context of recent related works. 

%While the information bottleneck can be intuitively understood as optimizing a trade-off between a rate and distortion function, this arises with some nuances from rate-distortion theory.
%With our proposed method in mind, we review rate-distortion theory and its application in several recent works.

Given a source distribution $X \sim \qd$ and a distortion function $d : \mathcal X \times \mathcal Z \mapsto \mathbb{R}^{+}$ over samples and their codes $Z$, the rate-distortion function is defined as an optimization over conditional distributions $q(\vz|\vx)$:
\be
R(D) & = \min_{q(\vz|\vx)} I_{q}(X;Z) \\
& \text{ subj  }\mathbb{E}_{\qd q(\vz|\vx)} d(\vx, \vz) \leq D \label{eq:rd}
\ee
It is common to optimize an unconstrained problem by introducing a Lagrange multiplier $\beta^{-1}$ which, at optimality, reflects the tradeoff between compression and fidelity as the slope of the rate-distortion function at $D$, i.e. $\beta^{-1} = -\frac{\partial R}{\partial D}$:
\be
\mathcal L = \max_{\beta} \min_{q(\vz|\vx)} I_{q}(X;Z) + \beta^{-1} \, \big( \mathbb{E}_{\qd q(\vz|\vx)} d(\vx, \vz) - D \big) \nonumber %\label{eq:rdlagr}
\ee
Eq. \ref{eq:problemdef} suggests the cross entropy reconstruction loss as a distortion measure, so that $d(\vx, \vz) = - \log \dec$.  We can then observe the equivalence between the rate-distortion optimization and our problem definition, as only the tradeoff between rate and distortion affects the characterization of solutions.  \cite{alemi2018fixing} also analyse this distortion measure in the context of  upper and lower bounds on $\iq$:
\benn
H_{q}(X) -  \eq \log \dec \leq I_q \leq \kl [ \enc || r(\vz) ]
\eenn
With the data entropy as a constant, minimizing the cross entropy distortion corresponds to the variational information maximization lower bound of \citet{agakov2005variational}.  
The upper bound is identical to the decomposition in Eq. \ref{eq:mi_ub}, and it can be shown that $\qz = \argmin_{r} \kl [\enc || r(\vz)]$ using the non-negativity of the KL divergence.  Thus, any marginal distribution $r(\vz)$ will provide an upper bound on mutual information with a gap of $\kl [ \qz || r(\vz)].$ 

Several recent works have observed this fact and considered `learned priors' or marginal approximations \cite{chen2016variational, tomczak2017vae, alemi2018fixing} that seek to match $\qz$, thereby reducing $\kl [ \qz || r(\vz)]$ and tightening our bounds.   From this perspective, a static Gaussian prior can be seen as providing a particular and possibly loose marginal approximation \cite{gao2018auto, alemi2018fixing}.  The analysis in \citet{rosca2018distribution} suggests that the marginal divergence can indeed be significant for VAE models and their flow-based or adversarial extensions.  %This problem can be particularly severe for highly non-Gaussian datasets.
%In the absence of any domain-specific structure encoded in these priors or marginal approximations, we advocate using the tightest ELBO bound by focusing on the lossy compression goal of variational autoencoding.  Echo noise allows us to avoid loose bounds on mutual information by always working with the true encoding marginal. 

With this in mind, it is interesting to note the self-consistent equations which solve the variational problem above (see, e.g.  \citet{tishby2000information})
%We can draw connections with the generative modeling approach by observing the self-consistent equations which solve the variational problem in \eqref{eq:rdlagr} (see, e.g.  \citep{tishby2000information})
%The value of $\beta$ at optimality directly reflects the tradeoff between compression and fidelity by measuring the slope of the rate-distortion function at $D$, i.e. $\beta = -\frac{\partial R}{\partial D}$. Further, we can obtain an set of analytic self-consistent equations for the above variational problem in terms of $\beta$ (see, e.g. \citep{tishby2000information}):  
\be
q(\vz|\vx) &= \frac{q(\vz)}{Z(\vx, \beta)} \exp \big(-\beta^{-1} \, d(\vx, \vz) \big) \label{eq:rdsolution} \\
q(\vz) &= \int q(\vz|\vx) q(\vx) d{\vx} \nonumber
\ee
Notice that, regardless of the choice of distortion measure, our Echo noise channel enforces the second equation \textit{throughout} optimization by using the  encoding marginal as the `optimal prior.'  For our choice of distortion, the solution simplifies as in Theorem 1 of \citet{infolowerbounds}:  %
%We view the stochastic encoder as performing lossy compression of the data subject to fidelity constraints, a problem formally treated by rate-distortion theory \cite{cover}.  While previous works have made similar connections between rate-distortion and unsupervised learning \cite{alemi2018fixing, rezende2018taming, infolowerbounds} and are discussed in Section \ref{sec:related}, %
\be
q(\vz|\vx) &= \frac{q(\vz)p(\vx|\vz)^{1/\beta}}{Z(\vx, \beta)} \label{eq:rd_unsupervised}
\ee
This provides an interesting comparison with the generative modeling approach.  While the Evidence Lower Bound objective can be interpreted as performing posterior inference with prior $p(\vz)$ in the numerator, we see that the information theoretic perspective prescribes using the exact encoding marginal $q(\vz)$.  Indeed, we can interpret our tighter bound in Eq. \ref{eq:rd_bound} as corresponding to the likelihood under the generative model $p(\vx) = \int \qz \dec d{\vx}$.  The gap in the ELBO then becomes $\kl [\enc || \frac{q(\vz)p(\vx|\vz)}{Z(\vx)} ]$, encouraging the encoder to match the rate-distortion solution for $\beta = 1$.  

% MOVED TO RELATED

Several other recent works have drawn connections between maximum likelihood and rate-distortion theory.  \citet{infolowerbounds} demonstrate a symmetry between improvements in the marginal approximation and likelihood function.  \citet{rezende2018taming} analyse the latent space dynamics for solutions to the rate-distortion problem in Eq.~\ref{eq:rd}, although they use the traditional prior $p(\vz)$ and its upper bound on rate.  An `annealed posterior' similar to Eq. \ref{eq:rd_unsupervised} is considered from a Bayesian perspective in \citet{mandt2016variational}.
%For $\beta = 1$, the tighter likelihood bound discussed in Section \ref{sec:prelim} can be easily recovered.   


%\cite{alemi2018fixing} view tightening these bounds as targeting a specific value $\iq = C$, or a version of the equivalent distortion-rate problem.  The Lagrangian of this problem recovers the $\beta$-VAE objective \cite{higgins2017} for $r(\vz) = p(\vz)$ and the objective that we consider here:
%\benn
%\mathcal{L}_{\beta\mathrm{-VAE}} = \eq %\log \dec - \beta \kl[\enc || r(\vz) ] 
%\eenn




%Thus, for $Y = X$, the Information Bottleneck distortion of $\kl [q(y|\vx)|| q(y|\vz)]$ reduces to the conditional entropy $d(\vx, \vz) = \kl [q(\vx|\vx)|| q(y|\vz)] = -\mathbb{E}_{q} \log q(\vx | \vz)$.  The intractability of this posterior constitutes the primary difficulty of latent variable inference, so we may instead replace this distortion measure with $d(\vx, \vz) = -\mathbb{E}_{q} \log p(\vx | \vz)$, mismatched to the `ideal' task.  %by the quantity $\kl [ q(\vx | \vz) || p(\vx||\vz)]$ 
Existing models are usually trained with a static $\beta$ \cite{alemi2018fixing, higgins2017} or a heuristic annealing schedule \cite{bowman2016, burgess2018understanding}, which implicitly correspond to constant constraints.
However, setting target values for either the rate or distortion remains an interesting direction for future discussion. \citet{rezende2018taming} view the distortion as an intuitive user-specified choice, while \citet{zhao2018lagrangian} train a separate model to provide constraint values.  As both works show, specifying a constant and optimizing the Lagrange multiplier $\beta$ with gradient descent can improve performance.


%Finally, our method for calculating mutual information suggests exploring distortion measures for other applications. The Information Bottleneck method defines `relevant' information through another random variable $Y$, and can be seen as a special case of rate-distortion with distortion measure $\kl [q(y|\vx)|| q(y|\vz)]$ \cite{tishby2000information, banerjee2005clustering}.  Applied to supervised learning problems using an upper bound on the rate, \citet{alemi2016deep} show that Information Bottleneck can improve generalization and adversarial robustness. Further,  reinforcement learning can be framed in terms of rate-distortion using the theory of bounded rationality \cite{ortega2015information}.  Here, the agent trades off $I(A;S)$, the `deliberation cost' associated with choosing a state-dependent action, with a distortion measure which maximizes reward.

==> sections/related.tex <==
\section{Related Work}\label{sec:related}
% \textbf{Rate-Distortion:} Several other recent works have also drawn connections between maximum likelihood and rate-distortion.  \cite{infolowerbounds} demonstrate a symmetry between improvements in the marginal approximation and likelihood function.  \cite{rezende2018taming} analyse the latent space dynamics for solutions to the rate-distortion problem in \eqref{eq:rd}, although they use the traditional prior $p(\vz)$ and its upper bound on rate.  
% An `annealed posterior' similar to Eq. \eqref{eq:rd_unsupervised} is considered from a Bayesian perspective in \cite{mandt2016variational}.
% %For $\beta = 1$, the tighter likelihood bound discussed in Section \ref{sec:prelim} can be easily recovered.   


% %\cite{alemi2018fixing} view tightening these bounds as targeting a specific value $\iq = C$, or a version of the equivalent distortion-rate problem.  The Lagrangian of this problem recovers the $\beta$-VAE objective \cite{higgins2017} for $r(\vz) = p(\vz)$ and the objective that we consider here:
% %\benn
% %\mathcal{L}_{\beta\mathrm{-VAE}} = \eq %\log \dec - \beta \kl[\enc || r(\vz) ] 
% %\eenn




% %Thus, for $Y = X$, the Information Bottleneck distortion of $\kl [q(y|\vx)|| q(y|\vz)]$ reduces to the conditional entropy $d(\vx, \vz) = \kl [q(\vx|\vx)|| q(y|\vz)] = -\mathbb{E}_{q} \log q(\vx | \vz)$.  The intractability of this posterior constitutes the primary difficulty of latent variable inference, so we may instead replace this distortion measure with $d(\vx, \vz) = -\mathbb{E}_{q} \log p(\vx | \vz)$, mismatched to the `ideal' task.  %by the quantity $\kl [ q(\vx | \vz) || p(\vx||\vz)]$ 
% Existing models are usually trained with a static $\beta$ \cite{alemi2018fixing, higgins2017} or with a heuristic annealing schedule \cite{bowman2016, burgess2018understanding}, which implicitly correspond to constant constraints.
% However, setting target values for either the rate or distortion remains an interesting direction for future discussion. \cite{rezende2018taming} view the distortion as an intuitive user-specified choice, while \cite{zhao2018lagrangian} train a separate model to provide constraint values.  As both works show, specifying a constant and dynamically training the Lagrange multiplier $\beta$ with gradient descent can provide improved performance.

% Finally, our method for exactly calculating mutual information suggests exploring distortion measures for other applications. The Information Bottleneck method defines `relevant' information through another random variable $Y$, and can be seen as a special case of rate-distortion with distortion measure $\kl [q(y|\vx)|| q(y|\vz)]$ \cite{tishby2000information, banerjee2005clustering}.  Applied to supervised learning problems using an upper bound on the rate, \cite{alemi2016deep} show that Information Bottleneck can improve generalization and adversarial robustness. Further, our exact rate calculation could be relevant to reinforcement learning via the theory of bounded rationality \cite{ortega2015information}.  Here, the agent trades off $I(A;S)$, the `deliberation cost' associated with choosing a state-dependent action, with a distortion measure which maximizes reward. 


%\textbf{Mutual Information in Representation Learning: }
A number of recent works have argued that the maximum likelihood objective may be insufficient to guarantee useful representations of data \cite{infovae, alemi2018fixing}.  In particular, when paired with powerful decoders that can match the data distribution, Variational Autoencoders (VAEs) may learn to completely ignore the latent code \cite{bowman2016,chen2016variational}.  

To rectify these issues, a commonly proposed solution has been to add terms to the objective function that maximize, minimize, or constrain the mutual information between data and representation  \cite{infovae, zhao2018lagrangian, phuong2018mutual,braithwaite2018bounded, alemi2018fixing}.  However, justifications for these approaches have varied.  Further, since mutual information is intractable in general, different estimation methods have been employed in practice.  These include sampling \cite{phuong2018mutual}, autoregressive density estimation \citep{alemi2018fixing}, mixture entropy estimation \cite{kolchinsky2017nonlinear}, learned mixtures \cite{tomczak2017vae}, indirect optimization via other divergences \cite{infovae}, and a dual form of the KL divergence \cite{belghazi2018mine}.  
%Namely, this distortion measure matches the Variational Information Maximization lower bound on $iq$  \cite{agakov2004algorithm}, with a gap of $\kl [ q(\vx | \vz) || p(\vx||\vz)]$. \cite{alemi2018fixing} and \cite{rezende2018taming} also discuss this quantity as the distortion. 

%\textcolor{red}{ I would like Related Work to jump directly into rate-distortion for unsupervised learning:  Alemi, Achille, Ermon Lagrangian, InfoVAE...  possibly move this to motivation for intro }
%A number of recent works have argued that the maximum likelihood objective may be insufficient to learn "useful" or "interesting" representations of data \cite{alemi2018fixing,phuong2018mutual}.  In particular, when paired with powerful decoders that can match the data distribution, Variational Autoencoders (VAEs) may learn to completely ignore the latent code \cite{bowman2016}.  

%Adding mutual information terms or constraints to the objective function has been commonly proposed as a solution, but justifications for these objectives vary \cite{infovae,phuong2018mutual,braithwaite2018bounded,alemi2018fixing}.  Since mutual information is intractable in general, previous works have also employed a number of different approximation methods, including sampling \cite{phuong2018mutual}, density estimation with autoregressive models \citep{alemi2018fixing}, mixture entropy estimation \cite{kolchinsky2017nonlinear}, and indirect optimization via other divergences \cite{infovae}.  
\subsection{Comparison Methods} \label{sec:compare}
Among these approaches, the InfoVAE model of \citet{infovae} provides a potentially interesting comparison with our method.  The objective adds a parameter $\lambda$ to more heavily regularize the marginal divergence, and a parameter $\alpha$ to control mutual information.  After some simplification, the objective becomes:
\benn
\vspace{-.1in}
\mathcal{L}_{\mathrm{InfoVAE}} & = \eq \log \dec - (1-\alpha) \kl[ \enc || \pz ]\\
& - (\alpha + \lambda - 1) \kl [ \qz || \pz]
\eenn
\vskip -.1in
While it is difficult to directly optimize $\kl [ \qz || \pz]$, \cite{infovae} instead minimize the Maximum Mean Discrepancy (MMD) \cite{gretton2012kernel}, which will also be zero when $\qz = \pz$.  We choose to analyse the setting of $\lambda = 1000$ (as in the original paper) and $\alpha = 0$ (no information preference), so the objective becomes:
\benn
\vspace{-.1in}
\mathcal{L}_{\mathrm{InfoVAE}} & = \mathcal{L}_{ELBO} - 999 \, D_{\mathrm{MMD}} [ \qz || \pz]
\eenn
\vskip -.05in
%\textcolor{red}{ELBO + big MMD penalty} \\
The sizeable MMD penalty encourages $ \qz \approx \pz$, so that $\kl [\enc || \pz] \approx \kl [\enc || \qz] = \iq$.  Thus, the KL divergence term in the ELBO should more closely reflect a mutual information regularizer, facilitating comparison with the rate in Echo models.   
%Comparing InfoVAE with the regular VAE may then lend insight to the impact of tighter rate bounds on our autoencoders' ability to trade off compression and reconstruction.

Flow models, which evaluate densities on simple distributions such as Gaussians but apply complex transformations with tractable Jacobians, are another prominent recent development in unsupervised learning \cite{germain2015made, rezende2015variational, kingma2016improved, papamakarios2017masked}.  We compare against models using inverse autoregressive flow (IAF) in the encoder.  This is not a noise model, but can be seen as transforming the output of a Gaussian noise channel into an approximate posterior sample using an autoregressive network \cite{kingma2016improved}.  

We consider several marginal approximations alongside the IAF encoder, including a Gaussian prior with MMD penalty as described above (\textit{IAF+MMD}).  Masked autoregessive flow (MAF) \cite{papamakarios2017masked} models a similar transformation as IAF, but with computational tradeoffs suited to density estimation (\textit{IAF-MAF}).   Finally, we consider the VampPrior \cite{tomczak2017vae}, which estimates $\qz$ as a mixture of Gaussian encoders $\frac{1}{K} \sum_{k} q(\vz|\mathbf{u}_k)$ conditioned on a set of learned `pseudo-inputs' $\mathbf{u}_k \in \mathbb{R}^{d_x}$ (\textit{IAF-Vamp}).
 



% and masked autoregressive flow  (MAF) \cite{papamakarios2017masked} as a marginal approximation, identical to the model evaluated in \cite{alemi2018fixing}.   For additional comparisons, we use an IAF encoder in the InfoVAE setting above, with a standard Gaussian marginal and MMD penalty. 


% We again add a sizeable MMD penalty to force the IAF samples to resemble a standard Gaussian, and examine the relative weighting of mutual information and marginal mismatch in these models.

%This not only allows us to measure the benefit of mutual information regularization, but also may ease the task of the MAF estimator, which must transform encoding samples to high density regions of a standard Gaussian.  





